Correlations of the squares of the Riemann zeta on the critical line

We compute the average of a product of two shifted squares of the Riemann zeta on the critical line with shifts up to size $T^{3/2-\varepsilon}$. We give an explicit expression for such an average and derive an approximate spectral expansion for the error term similar to Motohashi's. As a consequence, we also compute the $(2,2)$-moment of moment of the Riemann zeta, for which we partially verify (and partially refute) a conjecture of Bailey and Keating.

==> explicit.tex <==

\label{section:explicit}

Now we would like to evaluate the diagonal $m=n$ and the off-diagonal $m\neq n$ contributions separately. The former is quite simple, while the latter constitutes the bulk of the computation.

When evaluating the off-diagonal term, there are two distinct regimes. When $\delta$ is small, the integral
\begin{equation*}\label{eq:wJkappa}
    \int W(t)J_{\delta}(nm,t) \big(\frac{m}{n}\big)^{it}\kappa(t) dt
\end{equation*}
behaves similarly to the Fourier transform of $WJ_{\delta}$ at $\eta(T) = \log m/n + \phi^\prime(T)$. When $\delta$ is large, the main contribution comes from the stationary point instead. In both cases the off-diagonal term computation relies on bounds for the error term in the correlations of the divisor function $d(n) = \sum_{k|n} 1$, or
\[
\sum_{n\le X} d(n)d(n+r)\,.
\]

\subsection{Diagonal term}

\begin{lem}\label{lem:diagJI} Suppose $\delta \ll T/\sqrt{Q}$, then
    \[
    \sum_{n\ge 1} \frac{d^2(n)}{n^{1-i\delta}} \int_0^{+\infty} W(t) \kappa(t) J_{\delta}(n^2,t) dt = \sum_{n\ge 1} \frac{d^2(n)}{n^{1-i\delta}} \int_0^{+\infty} W(t) \kappa(t) I(t/2\pi n) dt + O(T^\varepsilon\delta Q^{-1/2})\,.
    \]
\end{lem}
\begin{proof}
Recall that for $x,t,\delta>0$ and $\xi = \log \frac{t(t+\delta)}{4\pi^2 x}$
\begin{equation}
    J_\delta (x,t) = \frac{1}{2\pi i} \int_{(1)} \brackets{\frac{t(t+\delta)}{4\pi^2 x}}^z G(z)\frac{dz}{z} = \sqrt{Q} \int_{-\infty}^{\xi} e^{-\frac{Q}{4}y^2} dy\,,
\end{equation}
then
\[
J_\delta (n^2,t) - I(t/2 \pi n) = \frac{1}{2\pi i} \int_{(1)} \brackets{\frac{t}{2\pi n}}^{2z}\brackets{e^{z\log \frac{t+\delta}{t}}-1} G(z)\frac{dz}{z}\,.
\]
We have a convergent series
\[
e^{z\log \frac{t+\delta}{t}}-1 = z\log \frac{t+\delta}{t} + \frac{z^2}{2}\log^2 \frac{t+\delta}{t} + \ldots
\]
with $j$-th term of size
\[
\frac{z^j}{j!} \log^j \frac{t+\delta}{t} \ll \frac{T^\varepsilon Q^{j/2}\delta^j}{j!T^j}\,,
\]
provided that $t \asymp T$ and $z \ll Q^{1/2}T^\varepsilon$. Thus similarly to Lemma \ref{lem:Bbound}
\[
J_\delta (n^2,t) - I(t/2 \pi n) \ll \frac{\delta}{T} e^{-\frac{Q}{8} \log^2 \frac{t}{2\pi n}}\,,
\]
and using that $W(t)$ restricts us to $t \asymp T$,
\[
\begin{aligned}
\sum_{n\ge 1} \frac{d^2(n)}{n^{1-i\delta}} \int_0^{+\infty} W(t) \kappa(t) (J_\delta(n^2,t)-I(t/2\pi n)) dt \ll
\frac{\delta}{T}\sum_{n\ge 1} \frac{d^2(n)}{n} \int_0^{+\infty} |W(t)|e^{-\frac{Q}{8} \log^2 \frac{t}{2\pi n}} dt \ll \\
\frac{\delta}{T}\sum_{n\ll T^2} \frac{d^2(n)}{n} \frac{T^{1+\varepsilon}}{\sqrt{Q}}\ll \frac{T^\varepsilon \delta}{\sqrt{Q}}\,
\end{aligned}
\]
as required.
\end{proof}

\begin{thm}[Diagonal term]\label{thm:diag} Let $W$ be an infinitely differentiable function supported on $[T_1,T_2]\subseteq [T,2T]$ chosen with parameter $\Delta$. Let $\delta \ll T^{2-\varepsilon}$. Then
\begin{equation*}
    \begin{aligned}
       2 \re \sum_{n\ge 1} \frac{d^2(n)}{n^{1-i\delta}} \int_0^{+\infty} W(t) & \kappa(t) J_{\delta}(n^2,t) dt = \\
      % & 2 \re \res_{s \in \{0,i\delta\}} L(1+s) \frac{\tilde{W}(1+s) G(s-i\delta)}{s-i\delta} + O(T^{1/2+\varepsilon}) = \\
      & 2T \re(F(T_2) - F(T_1)) +O(T^{\varepsilon}\Delta + T^{1+\varepsilon}/Q)\,,
    \end{aligned}
    % T^{1/2} + \min\{T/\delta,\Delta + T\delta/Q\}
\end{equation*}
where
\[
F(X) = \res_{s \in \{0,i\delta\}} \frac{\zeta^4(1+s)}{\zeta(2+2s)}  \frac{(X/2\pi)^s}{s-i\delta}\,.
\]
In fact, if $\delta \gg T^{1/3}$, the whole expression is $O(T^{2/3+\varepsilon})$.
\end{thm}
\begin{proof} First, recall that
 \begin{equation*}
     \kappa (t) = \chi\brackets{1/2-it} \chi\brackets{1/2 + i(t +\delta)} = e^{i\phi(t)}(1+ O(|t|^{-1}))\,,
\end{equation*}
where
\begin{equation*}
    \phi(t) = t\log \frac{t}{2\pi e} - (t+\delta)\log \frac{t+\delta}{2\pi e}
\end{equation*}
and $\phi^\prime(t) = \log t - \log (t+\delta)$. Second, notice that both $W(t)$ and $J_\delta (nm,t)$ are bounded real functions. Hence for $\delta \gg T^{\varepsilon}$ and $ n^2 \ll T^4$ the oscillation lemma gives
\[
\begin{aligned}
\int_0^{+\infty} \kappa(t) W(t) J_{\delta}(n^2,t) dt= \int_1^{+\infty} e^{i\phi(t)}(1+ O(1/|t|) W(t)  J_{\delta}(n^2,t) dt + O(1) \ll \\
 \frac{\max |W(t)J_{\delta}(n^2,t)|}{\min_{t \asymp T} |\phi^\prime(t)|}  + 1 \ll \brackets{\log \frac{T+\delta}{T}}^{-1} + 1 \ll T\delta^{-1} + T^{\varepsilon}\,.
\end{aligned}
\] 
If $n^2 \gg T^4$, we observe that
\[
J_\delta(nm,t) \ll e^{-\frac{Q}{4} \log^2\frac{t(t+\delta)}{4\pi^2n^2}} \ll e^{-\frac{Q}{8} \log^2 n}
\]
making the contribution of such $n$ negligible. Thus, the contribution of the diagonal term is bounded by
\begin{equation*}
   \int \kappa(t) W(t) \sum_{n\ge 1} \frac{d^2(n)}{n^{1-i\delta}} J_{\delta}(n^2,t) dt \ll T^{\varepsilon} \brackets{T\delta^{-1} + 1} \sum_{n\ll T^2} \frac{d^2(n)}{n}  \ll T^{\varepsilon} \brackets{T\delta^{-1} + 1} \,. 
\end{equation*}

On the other hand, if $\delta\ge 0$ is relatively small, say $\delta \ll Q^{1/2-\varepsilon}$, then by Lemma \ref{lem:diagJI}
\[
    \int_0^{+\infty} W(t) \kappa(t) \sum_{n\ge 1} \frac{d^2(n)}{n^{1-i\delta}}  J_{\delta}(n^2,t) dt =  \int_0^{+\infty} W(t) \kappa(t) \sum_{n\ge 1} \frac{d^2(n)}{n^{1-i\delta}} 
 I(t/2\pi n) dt + O(T^{1/2+\varepsilon})\,.
    \]
Further,
\[
\begin{aligned}
    \int_0^{+\infty} & W(t) \kappa(t) \sum_{n\ge 1} \frac{d^2(n)}{n^{1-i\delta}} I(t/2\pi n) dt = \\ 
    & \int_0^{+\infty} W(t) \sum_{n\ge 1} \frac{d^2(n)}{n} 
 \brackets{\frac{t}{2\pi n}}^{-i\delta}\brackets{1 + O(\delta^2/|t|)} I(t/2\pi n) dt = \\
   &  \int_0^{+\infty} W(t) \sum_{n\ge 1} \frac{d^2(n)}{n} \brackets{\frac{t}{2\pi n}}^{-i\delta} I(t/2\pi n) dt + O(\delta^2 T^\varepsilon)\,.
\end{aligned}
\]
Here we essentially have the Mellin transform of $W(t) I(t/2\pi n)$, while $I(w)$ is in turn the inverse Mellin transform of $G(z)$. Denote the Mellin transform of $W$ by
\[
\tilde{W}(s) = \mathcal{M}W(s) = \int_0^\infty x^{s-1}W(x) dx\,,
\]
and set $L(s) = \zeta^4(s)/\zeta(2s)$. Then
% using Lemma \ref{lem:smallprep}
\begin{equation*}
    \begin{aligned}
    \int_0^{+\infty}  W(t) \sum_{n\ge 1}  \frac{d^2(n)}{n} \brackets{\frac{t}{2\pi n}}^{-i\delta} I(t/2\pi n) \ll
    % & \int_0^{+\infty} |W(t)| \sum_{n\ge 1}  \frac{d^2(n)}{n} \int_{-\infty}^{\infty} \brackets{\frac{t}{2\pi n}}^{2} |G(1+iy)| \frac{dy}{1+|y|} \ll 
    T^3 \sum_{n\ge 1} \frac{d^2(n)}{n^3} \int_{-\infty}^{\infty}  \frac{|G(1+iy)|dy}{1+|y|}
    \end{aligned}
\end{equation*}
is absolutely convergent, thus applying Fubini's theorem (or the Mellin convolution theorem),
\begin{equation*}
    \begin{aligned}
    \ \int_0^{+\infty} W(t) \sum_{n\ge 1}  \frac{d^2(n)}{n}  \brackets{\frac{t}{2\pi n}}^{-i\delta} I(t/2\pi n) dt = \\
 \frac{1}{2\pi i}\int_{(2)} L(1+z-i\delta) \tilde{W}(1+z-i\delta)  \frac{G(z/2)}{(2\pi)^{z-i\delta}z}dz = \\
\frac{1}{2\pi i}\int_{(2)} L(1+s) \tilde{W}(1+s)  \frac{G((s+i\delta)/2)}{(2\pi)^{s}(s+i\delta)}ds\,.
        % \res_{s \in \{0,i\delta\}} L(1+s) \frac{\tilde{W}(1+s) G((s+i\delta)/2)}{(2\pi)^{s}(s+i\delta)} + O(T^{1/2+\varepsilon})\,.
    \end{aligned}
\end{equation*}
Note that $\tilde{W}(1+s) = \int_0^{+\infty}x^s W(x) dx$ is well-defined for $\re s > -1$ with
\[
\tilde{W}(1+s) \ll \frac{T^{1+\re s}}{1+|\im s|}\,.
\]
Shifting the contour to $\re s = -1/2$ and applying standard bounds $\zeta(\sigma+it) \ll (1+|t|)^{1/6+\varepsilon}$ and $\zeta(1+it) \gg \log\log (2+|t|)$, 
\[
\frac{1}{2\pi i}\int_{(2)} L(1+s) \tilde{W}(1+s)  \frac{G((s+i\delta)/2)ds}{(2\pi)^{s}(s+i\delta)} = \res_{s \in \{0,-i\delta\}} \frac{L(1+s) \tilde{W}(1+s) G((s+i\delta)/2)}{(2\pi)^{s}(s+i\delta)} + O(T^{1/2+\varepsilon})\,.
\]
At $s = -i\delta$ we have $G(0) = 1$ and
\[
\tilde{W}(1\pm i\delta) - \int_{T_1}^{T_2} x^{\pm i\delta} dx = \int_0^{+\infty} x^{\pm i\delta}W(x) dx - \int_{T_1}^{T_2} x^{\pm i\delta} dx \ll \Delta T^\varepsilon \,.
\]
Thus if $\delta \neq 0$, then $s=-i\delta$ is a simple pole with residue
\[
\begin{aligned}
    \res_{s =-i\delta} \frac{L(1+s) \tilde{W}(1+s) G((s+i\delta)/2)}{(2\pi)^{s}(s+i\delta)} =  \frac{L(1-i\delta) \tilde{W}(1-i\delta) G(0)}{(2\pi)^{-i\delta}} = \\
    \res_{s =-i\delta} \frac{L(1+s)  (X/2\pi)^s}{(s+i\delta)(1+s)}\bigg\vert_{T_1}^{T_2} + O(\Delta T^\varepsilon)\,.
\end{aligned}
\]
Further, at $s=0$ we have $G(i\delta/2) = 1 + O(\delta^2/Q)$, and for any $l \in \ZZ^{\ge 1}$
% $s = 0$ is a pole or order $4$ or $5$ (if $\delta=0$), and
\[
\tilde{W}^{(l)}(1) = \int_{T_1}^{T_2} (\log x)^l dx + O(\Delta T^\varepsilon),\quad G^{(l)}(i\delta/2) \ll_l \delta/Q\,,
\]
hence
\[
\res_{s = 0 } \frac{L(1+s) \tilde{W}(1+s) G((s+i\delta)/2)}{(2\pi)^{s}(s+i\delta)} =  \res_{s = 0} \frac{L(1+s)  (X/2\pi)^s}{(s+i\delta)(s+1)}\bigg\vert_{T_1}^{T_2} + O(\Delta T^\varepsilon + T^{1+\varepsilon}\delta Q^{-1})\,.
\]
% Then
% \[
%  \frac{1}{2\pi i}\int_{(2)} L(1+s) \tilde{W}(1+s)  \frac{G((s+i\delta)/2)ds}{(2\pi)^{s}(s+i\delta)} = 
%  \res_{s \in \{0,-i\delta\}}  \frac{L(1+s)(X/2\pi)^s}{(s+1)(s+i\delta)}\bigg\vert_{T_1}^{T_2} + T^{\varepsilon}O(\Delta + T\delta/Q)\,.
% \]
Taking the minimum between two regimes yields the statement of the theorem.
% If $\delta = 0$ we only have one pole of order $5$ with residue
% % \[
% % \res_{s = 0} \frac{L(1+s) \tilde{W}(1+s) G(s/2)}{(2\pi)^{s}s}
% % \]
% \begin{equation*}
%  \text{Res}_{s=0} \frac{\zeta^4(1+s) (T/2\pi)^s}{\zeta(2+2s)s(s+1)}\,.
% \end{equation*}
% corresponding to the diagonal term of the $4$-th moment of the Riemann zeta. 
\end{proof}



% =----------------
\subsection{Off-diagonal term for small shifts}

In this subsection we consider $0 \le \delta \ll T^{1/2-\varepsilon}$, and assume that $T^{\varepsilon} \delta \ll Q \ll T$ as well as $\Delta Q^{1/2} \ll T$. In fact, we can set $\Delta Q^{1/2} = T$, though this is not necessary. Finally, set
\begin{equation}
    W(t)
    = F_{\Delta} \ast \II_{[T_1,T_2]}(t)\,,
\end{equation}
where
\[
F_{\Delta}(t) =  (\sqrt{\pi} \Delta)^{-1} e^{-t^2/\Delta^2}\,.
\]
Now let us simplify \eqref{eq:wJkappa} in a manner similar to Lemma \ref{lem:truncated}. The error term for the fourth moment of the Riemann zeta is at least of size $T^{1/2+\varepsilon}$, so we do not expect to be able to capture any terms of smaller size making this a natural first step.

In this range let us show that we can replace $J_{\delta}(mn,t)$ by
\begin{equation}\label{eq:iw}
    I(w) := \frac{1}{2\pi i} \int_{(1)} w^{2z} G(z) \frac{dz}{z}\,,
    % = \mathcal{M}^{-1}F(1/w)\,
\end{equation}
where $w=t/2\pi n$. 
% $F(z) = G(z/2)/z$ and 
% --------------------

\begin{lem}\label{lem:smallprep} 
% Let $W$ be a Schwartz function (approximately) compactly supported on $[T_1,T_2]$, where $T_j \asymp T$. 
Let $\delta \ll T^{1/2- \varepsilon}$ and
\[
U_{\delta}(x) = 2\pi \int W(2\pi x w) e^{2\pi i r w} w^{-i\delta} I(w) dw \,.
\]
Then 
\begin{equation*}
\begin{aligned}
\sum_{n\neq m}\frac{d(n)d(m)}{n^{1/2}m^{1/2-i\delta}}\int \big(\frac{m}{n}\big)^{it} W(t) \kappa(t) J_{\delta}(nm,t) dt
     =   2 \re \sum_{n,r \ge 1}
   d(n)d(n+r) U_\delta(n) + 
   O(\frac{T^2}{\Delta^2} +\delta^{3/2})\,.
\end{aligned}
\end{equation*}
\end{lem}
% -----------
\begin{proof}
We start with considering the integral
\begin{equation}\label{eq:genJI}
    \int \big(\frac{m}{n}\big)^{it} W(t) \kappa(t) (J_\delta(nm,t)-I(t/2\pi n)) dt\,.
\end{equation}
Let $f(y) = \mathcal{F} (\kappa(J_\delta(nm,\cdot) - I))(y)$, then by the Fourier convolution theorem
\[
\int \big(\frac{m}{n}\big)^{it} W(t) \kappa(t)  (J(nm,t)-I(t/2\pi n)) dt = (\hat{W} \ast f)(-\frac{1}{2\pi} \log \frac{m}{n})\,.
\]
Set $a := 2\pi n$ and $\eta_y(x) := 2\pi y + \phi^\prime(x)$. When $y = \frac{1}{2\pi}\log m/n$ we will omit the index and simply write $\eta(x)$. 

First, observe that
\[
\frac{t(t+\delta)}{4\pi^2 mn} = \frac{t^2}{4\pi^2 n^2} \frac{1+\delta/t}{1+ (m-n)/n}\,
\]
and
\[
\eta(t) =  \log \frac m n + \log \frac{t}{t+\delta} = \log \frac{1 + (m-n)/n}{1 + \delta/t}\,.
\]
Let $w = t/2\pi n = t/a$, then
\begin{equation*}
    J_\delta(nm,t) = \frac{1}{2\pi i} \int_{(1)} \brackets{\frac{t(t+\delta)}{4\pi^2mn}}^z G(z) \frac{dz}{z} = \frac{1}{2\pi i} \int_{(1)} w^{2z} e^{-z\eta(t)} G(z) \frac{dz}{z}\,,
\end{equation*}
and 
\begin{equation*}
        J_\delta(nm,t)- I(t/2\pi n) = \frac{1}{2\pi i} \int_{(1)} w^{2z} (e^{-z\eta(t)}-1) G(z) \frac{dz}{z}\,.
\end{equation*}
If $\eta(t) \ll Q^{-1/2}T^{-\varepsilon}$ we have
\begin{equation*}
    J_\delta(nm,t)- I(t/2\pi n) = -\frac{\eta(t)}{2\pi} \hat{G}(\frac{1}{\pi}\log \frac{t}{2\pi n}) (1 + E_1(t))\,,
\end{equation*}
where $E_1(t)$ is a convergent series in $t$ such that $E_1(t) \ll Q^{1/2}\eta^2(t)\ll Q^{-1/2}T^{-\varepsilon}$. The rate of decay of $\hat{G}$ restricts us to 
\[
\log \frac{t}{2\pi n} \asymp \frac{t-2\pi n}{2\pi n} \ll \frac{T^\varepsilon}{Q^{1/2}}\,.
\]
Change variables to $u=t-2\pi n = t - a$, then
\begin{equation}\label{eq:Fetaqsmall}
\begin{aligned}
f(-y) = \int e^{2\pi i yt} \kappa(t)   (J(nm,t)- I(t/a)) dt  = \\
- \frac{1}{2\pi} \kappa(a) \eta(a) e^{2\pi i ya} \int  e^{i\eta_{y}(a)u} \hat{G}(u/\pi a) (1+ E_2(u))du \,,
\end{aligned}
\end{equation}
where $E_2(u)$ is an absolutely convergent series in $u$, and 
\[
E_2(u) \ll \frac{\delta}{Q} + \frac{\delta}{nQ^{1/2}} + \frac{1}{Q^{1/2}}\,.
\]
Thus $f(-y)  \ll  a|\eta(a) G(i a \eta_{y}(a))|$, and applying the Fourier convolution theorem to \eqref{eq:genJI}
\begin{equation}\label{eq:JIsmall}
\begin{aligned}
    %  \int W(t) \big(\frac{m}{n}\big)^{it} \kappa(t)  (J_{\alpha,\beta}(nm,t)- I(t/a)) dt = 
     (\hat{W} \ast F)(\log m/n) \ll
          a|\eta(a)|\int |\hat{W}(\log m/n -y)  G(i a \eta_{-y}(a))| dy \ll \\
          \begin{cases}
           T^{\varepsilon} a|\eta(a)|, & \text{if $\eta(a) \ll T^{\varepsilon}(\Delta^{-1} + Q^{1/2}T^{-1})$}\,;\\
           T^{-a}, & \text{otherwise}\,.
           \end{cases}
\end{aligned}
\end{equation}
This follows from the fact that we need support of $\hat{W}(\log m/n -y)$ and $G(ia\eta_y(a))$ to overlap. Thus the contribution of $\log m/n \ll Q^{-1/2}T^{-\varepsilon}$ is
\begin{equation}\label{eq:etaqsmall}
    T^{\varepsilon} \sum_{nm \ll \tilde{T}^2}|\eta(a)| \II\{|\eta(a)| \ll T^{\varepsilon}(\Delta^{-1} + Q^{1/2}T^{-1})\} \ll \frac{T^{2+\varepsilon}}{\Delta^2} + Q T^{\varepsilon}\,.
\end{equation}
    On the other hand, if $\log m/n \gg Q^{-1/2}T^{-\varepsilon}$, integrating by parts,
\begin{equation}\label{eq:JIbig}
    \begin{aligned}
             &  \int W(t) \big(\frac{m}{n}\big)^{it} \kappa(t)  (J_{\delta}(nm,t)- I(t/2\pi n)) dt = \\
       & -\int \big(\frac{m}{n}\big)^{it} \kappa(t) \frac{1}{i\eta(t)} (W(J-I)(t))^\prime dt + \int W(t) \big(\frac{m}{n}\big)^{it} \kappa(t) (J-I)(t) \frac{\eta^\prime(t)}{i\eta^2(t)}dt\,.
    \end{aligned}
\end{equation}
Computing Fourier transforms of $W^\prime$ and $(J-I)^\prime$ we again observe that the first term is negligible when $\log m/n \gg Q^{-1/2} T^{-\varepsilon}$. The second term is bounded by $ \delta/(T^2\log^3 m/n)$ by the oscillation lemma. Its contribution is then
% \begin{equation}\label{eq:etaqbig}
%     \frac{1}{\log^2 m/n}\brackets{\frac{1}{\Delta} \wedge \frac{Q^{1/2}}{T} + \frac{\delta}{TQ^{1/2}}} \ll \frac{1}{\log^2 m/n}\brackets{\frac{1}{\Delta} + \frac{\delta}{TQ^{1/2}}}\,.
% \end{equation}
\begin{equation}\label{eq:etaqbig}
   \frac{\delta}{T^2} \sum_{nm \ll \tilde{T}^2} \frac{d(n)d(m)}{(nm)^{1/2}\log^3 m/n} \II\{\log m/n \gg Q^{-1/2} T^{-\varepsilon}\} \ll \frac{T^{\varepsilon} \delta Q}{T} \,.
\end{equation}
Thus the total error from \eqref{eq:etaqsmall} and \eqref{eq:etaqbig} is
% \begin{equation*}
% \begin{aligned}
%       \frac{T^2}{Q^{1/2}} \brackets{\frac{1}{\Delta}  + \frac{Q^{1/2}}{T}}^2 + TQ^{1/2} \brackets{\frac{1}{\Delta} \wedge \frac{Q^{1/2}}{T} + \frac{\delta}{TQ^{1/2}}} \ll \\
%       Q^{1/2} + \delta + \frac{T^2}{\Delta^2 Q^{1/2}} + \frac{TQ^{1/2}}{\Delta} \ll
%       T^{1/2} + \frac{T^{3/2}}{\Delta}\,.
% \end{aligned}
% \end{equation*}
\begin{equation}\label{eq:JItotal}
    T^\varepsilon\brackets{\frac{T^2}{\Delta^2} + Q + \frac{\delta Q}{T}}\,.
\end{equation}
Now let us similarly replace 
\begin{equation*}
    \frac{m^{i\delta}}{\sqrt{mn}} \int W(t) \big(\frac{m}{n}\big)^{it} \kappa(t)  I(t/2\pi n) dt\,,
\end{equation*}
with
\begin{equation}
    \frac{1}{n^{1-i\delta}} \int W(t) e^{itr/n} \brackets{t/2\pi}^{-i\delta} I(t/2\pi n) dt =  \frac{1}{n^{1-i\delta}} \int e^{i\omega(t)} W(t)I(t/2\pi n)  dt\,,
\end{equation}
where $r = m-n$ and $\omega(t) = tr/n - \delta \log t/2\pi$. Consider the difference
\begin{eqnarray*}
\int W(t)I(t/2\pi n)  \brackets{
 \big(\frac{m}{n}\big)^{i(t+\delta)} \kappa(t)  - e^{i\omega(t)}}  dt\ = 
        \int W(t)I(t/2\pi n) e^{i\omega(t)} (e^{ik(t)} - 1) dt\,,
\end{eqnarray*}
where
\[
k (t) = (t+\delta)\log (1 + r/n) - tr/n +  \phi(t) + \delta \log \frac{t}{2\pi} = (t+\delta)\log \frac{1 + \frac{r}{n}}{1+\frac{\delta}{t}} - t(\frac{r}{n} - \frac{\delta}{t})\,.
\]
Function $k(t)$ is divisible by the derivative of the new phase $\omega^\prime(t) = r/n - \delta/t$, thus integrating by parts
\begin{equation*}
    \begin{aligned}
        \int W(t)I(t/2\pi n) e^{i\omega(t)} (e^{ik(t)} - 1) dt = - \int e^{i\omega(t)} \brackets{W(t) I(t/2\pi n)\frac{e^{ik(t)} - 1}{i\omega^\prime(t)}}^\prime dt = \\
        - \int e^{i\omega(t)} \brackets{W(t) I(t/2\pi n)}^\prime \frac{e^{ik(t)} - 1}{i\omega^\prime(t)} dt -
    \int e^{i\omega(t)} W(t) I(t/2\pi n) \brackets{\frac{e^{ik(t)} - 1}{i\omega^\prime(t)}}^\prime dt\,.
    \end{aligned}
\end{equation*}
To evaluate the first integral, recall that for $W(t) = (F_{\Delta} \ast \II_{[T_1,T_2]})(t)$ and $I(w)$ defined as above
\begin{equation*}
    W^\prime(t) = F_{\Delta}(t-T_2) - F_{\Delta}(t-T_1); \quad \frac{d}{dt} I(t/2\pi n) = \frac{1}{\pi t}\hat{G}(\frac{1}{\pi} \log \frac{t}{2\pi n})\,.
\end{equation*}
Then
\begin{equation*}
    \int e^{i\omega(t)} F_\Delta(t- T_j) I(t/2\pi n)\frac{e^{ik(t)} - 1}{i\omega^\prime(t)} dt = 
\end{equation*}
and 
\begin{equation*}
\begin{aligned}
    \int e^{i\omega(t)} W(t) I^\prime (t/2\pi n)\frac{e^{ik(t)} - 1}{i\omega^\prime(t)} dt = \frac{1}{\pi} \int e^{i\omega(t)} W(t) \hat{G}(\frac{1}{\pi} \log \frac{t}{2\pi n}) \frac{e^{ik(t)} - 1}{i\omega^\prime(t)} \frac{dt}{t} 
    \end{aligned}
\end{equation*}

When $r/n \gg T^{-1/2-\varepsilon}$ we have $\omega(t) \gg r/n \gg T^{-1/2-\varepsilon}$, and by the oscillation lemma
\begin{equation}\label{eq:ktlarge}
    \int e^{i\omega(t)}  W(t) I(t/2\pi n) \brackets{\frac{e^{ik(t)} - 1}{\omega(t)}}^\prime dt \ll \frac{\delta n^3}{T^2 r^3}\,,
\end{equation}
otherwise if $r/n \ll T^{-1/2-\varepsilon}$, then $k(t) = o(1)$ and
\begin{equation*}
    \brackets{\frac{e^{ik(t)} - 1}{\omega(t)}}^\prime = -\frac{r}{2n} + O \brackets{\frac{r^2}{n^2} + \frac{\delta^2}{t^2}}\,
\end{equation*}
thus
\begin{equation*}
    \int e^{i\omega(t)}  W(t) I(t/2\pi n) \brackets{\frac{e^{ik(t)} - 1}{i\omega(t)}}^\prime dt = -\frac{r}{2n}\int e^{i\omega(t)}  W(t) I(t/2\pi n) dt + O\brackets{\frac{Tr^2}{n^2} + \frac{\delta^2}{T}}\,.
\end{equation*}



When $r/n \gg T^{-1/2}$ similarly to \eqref{eq:JIbig} by partial integration, where we again used the rate of decay of $\mathcal{F} W^\prime$ and $\mathcal{F} (J-I)^\prime$. When $\log m/n \ll T^{-1/2}$ and thus $\omega(t) \ll T^{-1/2}$ we have 
\begin{equation*}
    k(t) = -\frac{1}{2}\eta(t) \brackets{t\eta(t) + \delta(\frac{r}{n} + \frac{\delta}{t}) + O\brackets{\frac{(T+\delta)r^2}{n^2} +\frac{(T+\delta)\delta^2}{T^2}}} \ll 1\,.
\end{equation*}

The first integral similarly to \eqref{eq:JIsmall} is
\begin{equation*}
    \begin{aligned}
       \int e^{itr/n} t^{-i\delta} \brackets{W(t) I(t/2\pi n)}^\prime \frac{e^{ik(t)} - 1}{\omega(t)} dt \ll 
       I(\frac{T}{2\pi n})(T|\omega(T)| +  \frac{\delta r}{n} + \frac{\delta^2}{T}) \hat{W}(\omega(T)) +\\
       W(a) G(a \omega(a)) (a|\omega(a)| + |\delta| r/n + \delta^2/n)
    \end{aligned}
\end{equation*}

Summing over $m,n$ the above gives total error
\begin{equation*}
    \begin{aligned}
       \frac{\delta}{\tilde{T}} \sum_{nm \ll \tilde{T}^2}\frac{1}{(nm)^{1/2}}   \min\{\frac{\tilde{T}}{(1+\delta)^{1/2}}, \frac{\delta^{1/2}}{\log m/n}\} \II\{\log m/n \ll T^{-1/2}\} \ll T^{\varepsilon} + |\delta|^{3/2}\,
    \end{aligned}
\end{equation*}
and
\begin{equation*}
    \begin{aligned}
       \sum_{nm \ll \tilde{T}^2} \frac{1}{(nm)^{1/2}}(T|\eta(T)| + \frac{\delta^2}{\tilde{T}}) \II\{\eta(T) \ll \Delta^{-1} \log T \} \ll \frac{\tilde{T}^2}{\Delta^2} + \frac{\delta^2}{\Delta}\,;\\
       \sum_{nm \ll \tilde{T}^2} \frac{1}{(nm)^{1/2}}(n|\eta(a)| + \frac{\delta^2}{n}) \II\{\eta(a) \ll Q^{1/2}/n \wedge T^{-1/2}\} \ll \frac{\delta^{2}}{\tilde{T}^{1/2}}\,.
    \end{aligned}
\end{equation*}
This together with \eqref{eq:JItotal} implies the statement of the lemma.
% \[
% \beta + \frac{T^{3/2}}{\Delta} + T^{1/2} + \beta^{3/2} + (TQ)^{1/2} + \beta^{5/2} \brackets{\frac{1}{\Delta} + \frac{Q^{1/2}}{T}} \ll \frac{T^{3/2}}{\Delta} + T^{3/4}\,
% \]
% \begin{equation*}
%     \begin{aligned}
%       \frac{T^2}{\Delta^2 Q^{1/2}} + \frac{TQ^{1/2}}{\Delta} + \frac{T^{3/2}}{\Delta} + \beta^{3/2} + (TQ)^{1/2} + 
%     \end{aligned}
% \end{equation*}
% for $\delta \ll T^{1/2-\varepsilon}$ and $\Delta Q^{1/2} \ll T$\,.
% \begin{equation*}
%     T^{1/2} + \delta + \Delta\,.
% \end{equation*}
\end{proof}

Now let us evaluate the integral
\begin{equation*}
 2\pi\sum_{n,r \ge 1}
   d(n)d(n+r) \int W(2\pi nw) e^{2\pi i r w} w^{-i\delta} I(w) dw   
\end{equation*}
In order to use the asymptotic of divisor sum correlations, we need $|m-n|$ to be quite small. This is essentially the purpose of the parameter $\Delta$ for $W$.

There are two ways to approach this integral. We can choose $W$ and $G$ in such a way that the internal integral gives a smooth weight function of compact support and apply Motohashi's result in its full strength. Alternatively, we can use this result as a black box, but with a cleaner computation. For small $\delta$ we do the latter. 

\begin{lem}Let $0 \le \delta \ll T^{1/2-\varepsilon}$, and assume $\Delta^2 \delta \ll T^{2-\varepsilon}$. Let
\[
U(x) = 2\pi \int_{-\infty}^{+\infty} W(2\pi x w) e^{2\pi i r w} w^{-i\delta} I(w) dw \,,
\]
then
\[
U^\prime(x) = 
\]
\end{lem}

 \newpage
Let
\[
\sum_{n \le X} d(n) d(n+r) = S(X,r) + E(X,r)\,,
\]
where $S(X,r) = X \sum_{j=0}^2 b_j(r) \log^j X$ is the main term, and $E(X,r) = o(X)$ is the error term. Then we have the following.

\begin{lem}\label{lem:smallcorer}
% Let $W$ be a Schwartz function (approximately) supported on $[T_1,T_2]$, where $T_j \asymp T$. 
Let $0 \le \delta \ll T^{1/2-\varepsilon}$, and assume $\Delta^2 \delta \ll T^{2-\varepsilon}$. Let
\[
U(x) = 2\pi \int_{-\infty}^{+\infty} W(2\pi x w) e^{2\pi i r w} w^{-i\delta} I(w) dw \,.
\]
Then
\begin{equation*}
\begin{aligned}
    \sum_{n,r \ge 1}
   d(n)d(n+r) U(n)   = 
   - \sum_{r\ge 1} \int_0^\infty S(x,r) U^\prime(x) dx + O\brackets{\Delta + \frac{\delta \Delta^2}{T} +  \frac{T^{5/3}}{\Delta}}\,,
\end{aligned}
\end{equation*}
where $T^{5/3}/\Delta$ can be replaced with $T^{4/3}\Delta^{2/3}$ if $\Delta \delta \ll T^{1-\varepsilon}$.
\end{lem}
% ------------------------
\begin{proof}
Let $U(x)$ be as defined above, then $U(x)$ is smooth and for any $k \in \NN$
\[
U^{(k)}(x) = 2\pi \int_{-\infty}^{+\infty} (2\pi w)^k W^{(k)}(2\pi x w) e^{2\pi i r w} w^{-i\delta} I(w) dw\,. 
\]
Function $I(w)$ is similar to the indicator function on the interval $[1,+\infty)$, and $W^{(k)}(2\pi x w)$ is (approximately) supported on $[T_1/2\pi x, T_2/2\pi x]$. When $x \gg T^{1+\varepsilon}$, these intervals do not overlap. In particular, for $0 < w < 1$
\[
I(w) = \frac{1}{2\pi i} \int_{(1)}w^{2z} G(z) \frac{dz}{z} \ll e^{Q^{1/2} \log w}\,,
\]
thus when $x \gg T^{1+\varepsilon}$ for any $k \in \ZZ^{\ge 0}$
\[
U^{(k)}(x) \ll \brackets{\frac{T}{x}}^{\sqrt{Q}}\,.
\]
Then by partial summation
\begin{equation*}
%  \brackets{(S(x,r) + E(x,r)) U(x))\bigg\vert_1^\infty}
 \sum_{n \ge 1} d(n) d(n+r) U(n) = - \int_1^\infty (S(x,r) + E(x,r)) U^\prime(x) dx\,.
\end{equation*}
Set $\eta(x) = r/x - \delta/T$. For $W(t) = (F_{\Delta} \ast \II_{[T_1,T_2]})(t)$ we have
\[
W^\prime(t) = F_{\Delta}(t-T_2) - F_{\Delta}(t-T_1) = \frac{1}{\Delta\pi^{1/2}} e^{-\frac{(t-T_2)^2}{\Delta^2}} - \frac{1}{\Delta\pi^{1/2}} e^{-\frac{(t-T_1)^2}{\Delta^2}}\,.
\]
Substituting this into the integral and changing variables to $y = 2\pi x w-T_j$ each term gives
\begin{equation*}
\begin{aligned}
   \frac{4 \pi^{3/2}}{\Delta} \int e^{-\frac{(2\pi x w-T_j)^2}{\Delta^2}} & e^{2\pi i r w}  w^{1+i\delta} I(w) dw =
   \\
  & \frac{e^{\frac{iT_jr}{x}+i \phi(T_j)} }{\sqrt{\pi}\Delta x^{2+i\delta}} \int e^{-\frac{y^2}{\Delta^2}} e^{iy\eta(x)} (T_j+ y) I((T_j+y)/2\pi x)(1 + E(y))dy\,,
\end{aligned}
\end{equation*}
where $E(y) \ll y^2 \delta/T_j^2$ is a convergent series. Expanding $I(w)$ into a Taylor series near $T_j/2\pi x$ and computing the Fourier transform above we see that the above equals
\[
T_j\frac{e^{\frac{iT_jr}{x}+i \phi(T_j)}}{(2\pi)^{i\delta}x^{2+i\delta}}e^{-\frac{\Delta^2}{4}\eta^2(x)} I(T_j/2\pi x)(1+E_1(x))
\]
where $E_1(x)$ is again a convergent series in $x$ with
\[
E_1(x) \ll \frac{\Delta^2\delta}{\tilde{T}^2} + \frac{\Delta}{xT}\max_{|t-T_j|\le \Delta \log T} |\hat{G}(2\log t/2\pi x)|\,.
\]
% -------------------------------
This implies that
\begin{equation*}
    \begin{aligned}
       \int_1^\infty E(x,r) U^\prime(x) \ll \tilde{T} \int_1^\infty \frac{|E(x,r)|}{x^2} e^{-\frac{\Delta^2}{4}\eta^2(x)} I(T_j/2\pi x) dx \ll \\
      \tilde{T} \int_1^{3\tilde{T}} \frac{|E(x,r)|}{x^2} \II\{|\eta(x)| \le \log T/\Delta \} dx\,,
    \end{aligned}
\end{equation*}
which also restricts $r$ to the range $r \le \delta + \tilde{T}/\Delta$. If $\delta \ll \tilde{T}/\Delta$, we have
\begin{equation*}
\begin{aligned}
    \sum_{r\ge 1} \int_{r\Delta}^{3\tilde{T}} \frac{|E(x,r)|}{x^2} dx \ll  \int_{\Delta}^{3\tilde{T}} \sum_{r\le x/\Delta} |E(x,r)|\frac{ dx }{x^2} \ll
    \int_{\Delta}^{3\tilde{T}} \brackets{\frac{x^2}{\Delta}}^{2/3} \frac{ dx }{x^2} \ll \brackets{\frac{\tilde{T}}{\Delta^2}}^{1/3+\varepsilon}
\end{aligned}
\end{equation*}
using \eqref{eq:IMmeanexr}.
% the result of Ivic and Motohashi $\sum_{r\le R} |E(N,r)| \ll (R N)^{2/3+\varepsilon}$ for $R \ll N^{1/2-\varepsilon}$.
If $\tilde{T}/\Delta \ll \delta \ll (\tilde{T}/\Delta)^2$ and $\delta \ll T^{1/2-\varepsilon}$
\begin{equation*}
    \begin{aligned}
       \sum_{r\ge 1} \int_1^{3\tilde{T}} \frac{|E(x,r)|}{x^2} \II\{|\eta(x)| \le \log T/\Delta \} dx \ll \int_{T/\delta}^{3\tilde{T}}  \sum_{r = \frac{\delta x}{T} + O(\frac{x}{\Delta})} |E(x,r)| \frac{dx}{x^2} \ll \\
       \int_{T/\delta}^{3\tilde{T}}  \frac{x^{5/3}}{\Delta} \frac{dx}{x^2} \ll \frac{\tilde{T}^{2/3}}{\Delta}\,.
    \end{aligned}
\end{equation*}
% ------------------------------------
This is acceptable when $\Delta \gg \tilde{T}^{2/3}$. Finally, integrating by parts and using the oscillation lemma
\begin{equation*}
    \begin{aligned}
       \sum_{r \ge 1} \int_0^\infty S(x,r)e^{\frac{iT_jr}{x}} e^{-\frac{\Delta^2}{4}\eta^2(x)} I(T_j/2\pi x)E_1(x) \frac{dx}{x^{2+i\delta}}\ll \frac{\delta \Delta^2}{\tilde{T}} + \Delta\,.
    \end{aligned}
\end{equation*}
Combining these errors yields the statement of the lemma.
% Thus the total error is
% \[
% \Delta + \frac{\delta \Delta^2}{\tilde{T}} +  \frac{\tilde{T}^{5/3}}{\Delta}\,
% \]
% as required.
\end{proof}
% ---------------------

Now let us compute
\[
- \sum_{r\ge 1} \int_0^\infty S(x,r) U^\prime(x) dx\,.
\]
In fact, this is somewhat unnecessary since the essence of the problem is in bounding the error term, and we already know the Dirichlet series of $S(x,r)$. But let us finish the computation nonetheless.

We can remove $I$ and $W$ at the cost of an acceptable error and essentially follow \cite{conrey1996note}. However, let us do this using contour integration and Mellin transforms instead.
% --------------------------

\begin{thm}[Off-diagonal term]\label{thm:odsmall} 
% Let $W$ be an infinitely differentiable function (approximately) supported on the interval $[T,2T]$. 
Let $0 \le \alpha \le \beta \ll T^{3/2-\varepsilon}$ such that $\delta = \beta - \alpha \ll T^{1/2-\varepsilon}$. Let $\tilde{T}: = \sqrt{(T+\alpha)(T+\beta)} \ll T^{5/4-\varepsilon}$. Let
\[
h(z,s) = \frac{1}{\zeta(2+2s)}\brackets{ \zeta(1+z+s)\zeta(1-z+s) -\frac{2s\zeta(1+2z)}{s^2-z^2}}\,.
\]
Then
%  $\tilde{T}^{5/6}\delta^{1/4} \ll T^{1-\varepsilon}$. Then
\begin{equation*}
    \begin{aligned}
       2\re \sum_{n \neq m} \frac{d(n)d(m)}{n^{1/2+i\alpha}m^{1/2-i\beta}} \int W(t) \big(\frac{m}{n}\big)^{it} \kappa(t)  V_{\alpha,\beta}(nm,t) dt = \\
    %   2\re \frac{d^2}{dz^2}\frac{h_G(z,i\delta)}{z+1}\brackets{\frac{T_j e^{2\gamma}}{2\pi}}^z \bigg\vert_{z=0} + 
    %   O((T+\alpha)^{c+\varepsilon}) = \\
    \re(2T F(2T) - T F(T)) +  E(T)\,,
    \end{aligned}
\end{equation*}
where
\[
E(T) \ll \begin{cases}
\tilde{T}^{4/5+\varepsilon}, & \text{if $\delta\ll \tilde{T}^{1/3}$}\,;\\
\tilde{T}^{5/6}\delta^{1/4}, & \text{if $\tilde{T}^{1/3} \ll \delta\ll T^{1/2-\varepsilon}$}\,,
\end{cases}
\]
and
\[
       F(X) =  \frac{d^2}{dz^2}\frac{h(i\delta,s)}{z+1}\brackets{\frac{(X+\alpha)(X+\beta)}{4\pi^2}e^{2\gamma_0 }}^s \bigg\vert_{s=0} - \frac14 h(i\delta,0) \log^2 \frac{X+\alpha}{X+\beta}\,.
\]
We also recognise $h(z,s)$ as defined in \eqref{eq:moto_offdiag} and \eqref{eq:conjH2}.
\end{thm}



% \label{lem:smalldelta_explicit}
\begin{proof}
Without loss of generality set $\alpha = 0$. Let
\begin{equation*}
    U^\prime(x) = (2 \pi)^2 \int_0^\infty W^\prime(2\pi x w) e^{2\pi i r w} w^{1+i\delta} I(w) dw\,
\end{equation*}
as before. Let us show that $F(T)$ is given by
\begin{equation}
   T \sum_{r=1}^{\infty}\int_1^\infty S(x,r) e^{\frac{iTr}{x}+i \phi(T/x)}e^{-\frac{\Delta^2}{4}\eta^2(x)} I(T/2\pi x) \frac{dx}{x^2} \,,
\end{equation}
or equivalently after changing variables to $u = Tr/2\pi x$
\begin{equation*}
    \sum_{r=1}^\infty \frac{1}{r^{1-i\delta}} \int_0^{\infty} e^{2\pi i u}  S(Tr/2\pi u,r ) I(u/r) u^{-i\delta} e^{-\frac{\pi^2\Delta^2}{T^2}(u- \delta/2\pi)^2}du\,.
\end{equation*}
Let us rewrite this expression in a more convenient manner. First, let
\begin{equation*}
    Y(u,s) :=\frac{1}{2\pi i}  \int_{(2)}\zeta(1+s+z-i\delta)\zeta(z-s-i\delta) u^{z-i\delta-s-1} \frac{G(z)dz}{z} \,.
\end{equation*}
For further computations assume that $0<s<1$ is a real number. This does not affect the value of the integral and is only relevant when shifting the line of integration and picking up poles.

Second, using the expansion \ref{lem_conrey} we have
\begin{equation*}
    \begin{aligned}
      S(x,r) = x \sum_{k=1}^{\infty} \frac{\mu(k)}{k^2} \sum_{d|r} \frac{1}{d} \brackets{\brackets{\log \frac{xe^{2\gamma_0 -1}}{d^2k^2}}^2 + 1}  = 
      x \brackets{\sum_{k=1}^{\infty} \frac{\mu(k)}{k^{2}} \sum_{d|r}\frac{1}{d}} \frac{d^2}{ds^2}\frac{B^s}{s+1}\bigg\vert_{s=0} \,,
    \end{aligned}
\end{equation*}
where $B = xe^{2\gamma}/(dk)^2$. 

Using the above and changing the order of summation and integration due to absolute convergence rewrite the integral in question as
\begin{equation*}
\begin{aligned}
        %  r^{-(1+i\delta)} \int_0^{\infty} S(Tr/2\pi u,r ) I(u/r) e^{2\pi i u} u^{i\delta} e^{-\frac{\pi^2\Delta^2}{T^2}(u+ \delta/2\pi)^2} du = \\
            \sum_{r=1}^\infty \frac{1}{r^{1-i\delta}} \int_0^{\infty} e^{2\pi i u}  S(Tr/2\pi u,r ) I(u/r) u^{-i\delta} e^{-\frac{\pi^2\Delta^2}{T^2}(u- \delta/2\pi)^2}du = \\
  T \frac{d^2}{ds^2}\frac{A^s\zeta^{-1}(2+2s)}{s+1} \int_0^\infty e^{2\pi i u} e^{-\frac{\pi^2\Delta^2}{T^2}(u- \delta/2\pi)^2} Y(u,s) du\bigg\vert_{s=0}\,,
\end{aligned}
\end{equation*}
where $A = Te^{2\gamma_0}/2\pi$. Moving the line of integration to $(s+\varepsilon)$ we pick up the pole at $z=1+s+i\delta$ with residue
\begin{equation*}
    \begin{aligned}
       \zeta(2+2s)\frac{G(1+s+i\delta)}{1+s+i\delta}\int_0^\infty e^{2\pi i u} e^{-\frac{\pi^2\Delta^2}{T^2}(u- \delta/2\pi)^2} du\,,
    \end{aligned}
\end{equation*}
which gives error
\begin{equation*}
    \begin{aligned}
       T \frac{d^2}{ds^2}\frac{A^s}{s+1} \frac{G(1+s+i\delta)}{1+s+i\delta}\int_0^\infty e^{2\pi i u} e^{-\frac{\pi^2\Delta^2}{T^2}(u- \delta/2\pi)^2} du \bigg\vert_{s=0}\\,.
    \end{aligned}
\end{equation*}
If $\delta \gg Q^{1/2}$, then $G^{(l)}(1+i\delta) \ll |\delta/\sqrt{Q}|^{-b}$, otherwise when $\delta \ll Q^{1/2} \ll T/\Delta$
\[
\int_0^\infty e^{2\pi i u} e^{-\frac{\pi^2\Delta^2}{T^2}(u- \delta/2\pi)^2} du \ll \frac{T}{\Delta}e^{-T^2/\Delta^2}\,,
\]
so this is negligible in both cases.

Note that we initially set $r >0$. Combining with $r<0$ replaces $e^{2\pi i u}$ with $\cos(2\pi u)$. Changing the order of integration and essentially computing the Mellin transform of $\cos(2\pi u)$
\begin{equation*}
    \int_0^\infty \cos(2\pi u) u^{w-1} e^{-\frac{\pi^2\Delta^2}{T^2}(u- \delta/2\pi)^2}du = \frac{1}{(2\pi)^w} \cos (\pi w/2) \Gamma(w) + E(w)\,,
\end{equation*}
where $E(w) \ll (\Delta/T)^{1+\varepsilon}$, together with
\begin{equation*}
\begin{aligned}
   \frac{1}{(2\pi)^{w}}\zeta(w) \cos (\pi w/2) \Gamma(w) = \zeta(1-w)\,,
\end{aligned}
\end{equation*}
gives
\begin{equation*}
     \frac{1}{2\pi i}  \int_{(s+\varepsilon)}\zeta(1+s+z-i\delta)\zeta(1+s-z+i\delta) \frac{G(z)}{z}dz \,.
\end{equation*}
Moving the line of integration to $(0)$ with a small half-circle around $0$ gives $1/2$ of the residue at $z=0$, the residue at $z = s-i\delta$ and
\begin{equation}\label{eq:intrealpart}
     \re \frac{1}{2\pi i}  \int_b^\infty \zeta(1+s+iy+i\delta)\zeta(1+s-iy-i\delta) \frac{G(iy)}{y}dy = 0\,.
\end{equation}
Finally, the residues give
\begin{equation}
   \frac{1}{2} \zeta(1+s-i\delta)\zeta(1+s+i\delta) -\frac{\zeta(1+2s)G(s+i\delta)}{s+i\delta}\,.
\end{equation}
If $\delta \gg Q^{1/2}$, the second term is negligible. Otherwise
\begin{equation*}
    \re \frac{G(s-i\delta)}{s-i\delta} = \frac{2s}{s^2+\delta^2} + R(s)\,,
\end{equation*}
where $R(s)$ is an absolutely convergent series with largest terms
\[
\frac{s}{Q} + \frac{s \delta^2}{Q^2}\,.
\]
Hence we can replace $h_G$ with $h$ at the cost of an error of size $O(T/Q)$.

 Putting together errors from Lemmas \ref{lem:sweights}, \ref{lem:smallprep} and \ref{lem:smallcorer} we have error
 \begin{equation*}
     \frac{Q^{1/2}(\delta + Q^{1/2})}{\Delta} + \frac{\tilde{T}^2}{\Delta^2} + \Delta + |\delta|^{3/2} +  \frac{\delta\Delta^2}{\tilde{T}} + \frac{\tilde{T}^{4/3}}{\Delta^{2/3}} + \frac{\tilde{T}^{5/3}}{\Delta}\II\{\delta \Delta \gg \tilde{T}\}\,.
 \end{equation*}
 If $\delta \ll T^{1/3-\varepsilon}$ and $\tilde{T} \ll T^{5/4}$, set $Q = (\tilde{T}/\Delta)^2$ and $\Delta = \tilde{T}^{4/5}$, then this is $O(\tilde{T}^{4/5})$. If $T^{1/3} \ll \delta \ll T^{1/2}$, set $Q = (\tilde{T}/\Delta)^2$ and $\Delta = \tilde{T}^{5/6} /\delta^{1/4}$, which yields total error $O(\tilde{T}^{5/6}\delta^{1/4})$\,.
\end{proof}
% -----------------

% then summing over $r$ gives
% \begin{equation*}
%     \begin{aligned}
%       \sum_{r=1}^{\infty} \frac{S(Tr/2\pi u,r)}{r^{1+i\delta}}I(u/r) = 
%     \frac{T}{2\pi u} \frac{d^2}{dz^2}\brackets{\brackets{\frac{Te^{2\gamma_0-1}}{2\pi u}}^z
%     \frac{1}{\zeta(2+2z)}\sum_{k,l \ge 1} \frac{I(u/kl)}{k^{-z+i\delta}l^{1+z+i\delta}}} + \\
%     \frac{T}{2\pi u\zeta(2)}\sum_{k,l \ge 1} \frac{I(u/kl)}{k^{i\delta}l^{1+i\delta}}
%     \end{aligned}
% \end{equation*}
% Further,
% \begin{equation*}
%     \begin{aligned}
%       \sum_{k,l \ge 1} \frac{I(u/kl)u^{-z}}{k^{-z+i\delta}l^{1+z+i\delta}} = \frac{1}{2\pi i} \int_{(2)} \zeta(1+s+z+i\delta)\zeta(s-z+i\delta) u^{s-z} \frac{G(s) ds}{s}\,.
%     \end{aligned}
% \end{equation*}
% Integrating over $u$ then gives
% \begin{equation*}
%     \frac{1}{2\pi i} \int_{(2)} \zeta(1+s+z+i\delta)\zeta(s-z+i\delta) \Gamma(s-z+ i\delta) e^{\frac{\pi i}{2}(s-z+i\delta)} \frac{G(s) ds}{s}\,.
% \end{equation*}
% Using the functional equation of zeta and properties of the Gamma-function we have
% \[
% \frac{1}{2\pi i} \int_{(2)} \zeta(1+s+z+i\delta)\zeta(1-s+z-i\delta) \Gamma(\frac{1}{2} + \frac{s-z+i\delta}{2}) \Gamma(\frac{1}{2} - \frac{s-z+i\delta}{2}) e^{\frac{\pi i}{2}(s-z+i\delta)} \frac{G(s) ds}{s}
% \]
% Taking $z= \sigma$ real and shifting the integral to $(0)$ yields
% \begin{equation*}
%     \begin{aligned}
%       \frac{1}{2\pi i} \int_{|y| \ge a} |\zeta(1+\sigma+i(\delta+ y))|^2 \Gamma(\frac{1}{2} + \frac{s-z+i\delta}{2}) \Gamma(\frac{1}{2} - \frac{s-z+i\delta}{2}) e^{\frac{\pi i}{2}(s+i\delta)} \frac{G(iy) dy}{y}
%     \end{aligned}
% \end{equation*}

% \begin{lem}[Small shifts] Let $\alpha < \beta \ll T^{1-\varepsilon}$ with $\delta = \alpha-\beta$. Then
% \begin{eqnarray*}
%     % \int_{T}^{2T} |\zeta(1/2+it+i\alpha)\zeta(1/2+it+i\beta)|^2dt =\\ 
%     \mathcal{M}(T;\alpha,\beta) = 2 \re \sum_{\substack{m,n\\
%     |\eta(T)| \le  X}}
%     \frac{d(n)d(m)}{n^{1/2+i\alpha}m^{1/2-i\beta}} \brackets{\int_{\tau \wedge T}^{2T}  \brackets{\frac{m}{n}}^{it}\kappa(t) dt  +  F(T)} +\\
%     %  2 \sqrt{\delta} \re \sum_{\substack{m,n\\
%     % \frac{\log T}{\Delta} \ll |\eta(T)| \ll  \frac{\delta\log T}{T}}}
%     % \frac{d(n)d(m)}{|m-n|}  e^{i\delta \log |(m-n)/\delta|}  + \\
%     T^{\varepsilon}O(\delta  \Delta^2/T + \Delta)\,,
% \end{eqnarray*}
% where $X = X(T) = \log T(\frac{1}{\Delta} + \frac{\delta}{T})$.
% \end{lem}
% \begin{proof}
% Let $G_{\Delta}(t) =  (\sqrt{\pi} \Delta)^{-1} e^{-t^2/\Delta^2}$, and take
% \begin{equation}
%     W(t)
%     % = \frac{1}{\sqrt{\pi}{\Delta}} \int_{T}^{2T} e^{-(t-x)^2/\Delta^2} dx 
%     = G_{\Delta} \ast \II_{[T;2T]}(t)\,.
% \end{equation}
% Then
% \begin{equation}
%  \int_{ q} ^{\infty} W(t) \kappa(t) \brackets{\frac{m}{n}}^{it} dt   
% \end{equation}
% is essentially the Fourier transform of an analytic function. In particular, it is Schwarz, and decays faster than any power of $T$ once
% \[
% |\log m/n| \gg \log T (1/\Delta + \delta/T)\,.
% \]
% The contribution of $|q-jT| \ll \Delta \log T$ is $O(T^{\varepsilon}\Delta)$. For the remaining range let
% \begin{equation}
% F(X) = \frac{1}{i\eta(X)}e^{i\phi(X)} \brackets{\frac{m}{n}}^{iX}(\hat{G_\Delta} - 1)(\eta(X))\,,    
% \end{equation}
% then the above integral equals
% \begin{equation}
%     % \int_{T\wedge \tau} ^{2T} W(t) \kappa(t) \brackets{\frac{m}{n}}^{it} dt = 
%     \int_{\tau \wedge T}^{2T} \kappa(t) \brackets{\frac{m}{n}}^{it} dt  +  F(2T) -  F(\tau \wedge T) + O(\frac{\delta  \Delta^2}{T^2}\min \{\Delta, \eta(T)^{-1}\} )\,.
% \end{equation}
% % Using standard methods, one can show that the second term can be replaced with
% % \[
% % \hat{1}(\II_{[-\Delta\log T;\Delta \log T]} - 1)(\eta(X))
% % \]
% % at the cost of the error term of size $O(\Delta)$. 
% % If $\delta\Delta \gg T$, then in the regime $\log T/\Delta \ll \eta(T) \ll \delta \log T/T$ we have
% % \[
% % \int_{\tau}^{T} \kappa(t) \brackets{\frac{m}{n}}^{it} dt  +  F(T) = e^{is\log m/n + i \phi(s)} \frac{|s|}{\delta^{1/2}} + O (\delta/\eta^3(T) T^2 + T/\delta^{3/2})\,,
% % \]
% % where $s$ is the stationary point satisfying $\log m/n + \phi^\prime(s) = 0$. Note that
% % \[
% % s \log \frac{m}{n} +  \phi (s) + \beta \log m - \alpha \log n = \delta \log \frac{|\delta|}{2\pi e|m-n|}
% % \]
% % only depends on $m-n$. For $\eta(X) \ll \log T/\Delta$ we keep the integral as is. 
% If $|\eta(t)| \ge \log T/ \Delta$ for all $t \in [\tau, X]$, then
% \begin{eqnarray}
%     \int_{\tau}^{X} \brackets{\frac{m}{n}}^{it}e^{i\phi(t)} dt  = \frac{\brackets{\frac{m}{n}}^{it}e^{i\phi(X)}}{\eta(t)}\bigg\vert_{\tau}^{X} + \int_{\tau}^{X} \frac{\brackets{\frac{m}{n}}^{it}e^{i\phi(t)}}{\eta^2(t)} \phi^{\prime\prime}(t) dt\,.
% \end{eqnarray}
% Using the oscillation lemma for the second integral we obtain
% \begin{equation}
%  \sum_{\tau \le X}\frac{d(n)d(m)}{\sqrt{nm}} \frac{m^{i\beta}}{n^{i\alpha}} \int_{q}^{X} \frac{\brackets{\frac{m}{n}}^{it}e^{i\phi(t)}}{\eta^2(t)} \phi^{\prime\prime}(t) dt  \ll \frac{\delta \Delta^2}{X^{1-\varepsilon}} \wedge X^{1+\varepsilon}\,.   
% \end{equation}
% Finally, observing that
% \begin{eqnarray*}
%   M(T;\alpha,\beta) = \int_{-\infty}^{+\infty} W(t) |\zeta(1/2+it+i\alpha)\zeta(1/2+it+i\beta)|^2dt + O(T^{\varepsilon} \Delta)
% \end{eqnarray*}
% and summing over diadic intervals concludes the proof.
% \end{proof}



% \begin{lem}[Explicit formula] Let $\alpha < \beta \ll T^{2/3-\varepsilon}$ with $\delta = \alpha-\beta$. Then
% \begin{eqnarray*}
% \mathcal{M}_{2,2}(T;\alpha,\beta) = \sum_{n\le T/2\pi} \frac{d^2(n)}{n^{1+i\delta}} \int_{2\pi n}^T \kappa(t) dt + 
% % \sum_{r=0}^{\infty} \int S^\prime(x,r) \int_{\tau \wedge T}^{2T} \kappa(t) \brackets{\frac{x+r}{x}}^{it} dt dx + O (\Delta + T^{5/3}/\Delta + \delta \Delta^2/T )
% e^{i\phi(T)} \sum_{r\neq 0} \frac{1}{r} \int  e^{i\frac{(T+\beta)r}{x}} \brackets{\frac{S(x,r)}{x^{i\delta}}}^\prime dx +\\ O(T^{5/6+\varepsilon}(1+\delta^{1/3}/T^{1/18}))\,.
% \end{eqnarray*}
% \end{lem}
% \begin{proof}
% Suppose $m=n$, then the corresponding part of the sum is
% \begin{eqnarray}
%  \sum_{n\le T/2\pi} \frac{d^2(n)}{n^{1+i\delta}} \int_{2\pi n}^T \kappa(t) dt\,.
% \end{eqnarray}
% Let $m = n + r$ with $r \neq 0$ and denote
% \begin{equation}
% G(x) := \frac{1}{x^{1/2+i\alpha}(x+r)^{1/2-i\beta}}\brackets{\int_{\tau }^{T} \kappa(t) \brackets{\frac{x+r}{x}}^{it} dt  +  F(T) }\,.    
% \end{equation}
% We have
% \[
% G(x) \ll \frac{1}{x}\brackets{\min\{\frac{T}{(1+\delta)^{1/2}}, \frac{x\sqrt{1 +\delta}}{r}\} +  \min \{\Delta^2 \eta(T), \eta^{-1}(T)\}}\,,
% \]
% and
% \begin{equation}
%  G^\prime(x)  = \frac{e^{i\phi(T)} \brackets{\frac{m}{n}}^{iT}}{x^{2+i\delta}} \brackets{- \brackets{T + \frac{\Delta^2 r}{x}}e^{-\frac{\Delta^2}{4}\eta^2(T)} + \frac{\delta(e^{-\frac{\Delta^2}{4}\eta^2(T)} - 1)}{T\eta^2(T)}} + O\brackets{ \frac{Tr^3}{x^5\eta(T)}} \,.   
% \end{equation}
% If $\delta\Delta \gg T$, then in the range $\log T/\Delta \ll \eta(T) \ll \delta \log T/T$ we have
% \begin{equation}
% \int_{\tau}^{T} \kappa(t) \brackets{\frac{m}{n}}^{it} dt  +  F(T) = e^{is\log m/n + i \phi(s)} \frac{|s|}{\delta^{1/2}} + O (\delta/\eta^3(T) T^2 + T/\delta^{3/2})\,,    
% \end{equation}
% where $s$ is the stationary point satisfying $\log m/n + \phi^\prime(s) = 0$. Note that
% \begin{equation}
%   s \log \frac{m}{n} +  \phi (s) + \beta \log m - \alpha \log n = \delta \log \frac{|\delta|}{2\pi e|m-n|}  
% \end{equation}
% only depends on $m-n$. 

% Using partial integration we turn the sum over $n$ into
% \begin{eqnarray}
%  (S(x,r) + E(x,r) )  G(x) \bigg\vert_{A_r}^{B_r} - \int_{A_r}^{B_r}(S(x,r) + E(x,r)) G^\prime(x) dx\,,
% \end{eqnarray}
% where $A_r$ and $B_r$ come from the condition $\eta(T) \ll X(T)$. Using $E(x,r) \ll x^{2/3+\varepsilon}$, 
% \begin{equation}
%   \sum_r E(x,r) G(x) \bigg\vert_{A_r}^{B_r} \ll T^{2/3+\varepsilon}(1+\delta)^{1/2} + T^{5/3+\varepsilon}/\Delta\,.  
% \end{equation}
% For $\eta(T) \ll \log T/\Delta$ we have
% \begin{equation}
%   \sum_r\int_{A_r}^{B_r}E(x,r) G^\prime(x) dx \ll T^{5/3}/\Delta \,,  
% \end{equation}
% and for $\eta(T) \gg \log T/\Delta$ 
% \begin{equation}
%  \sum_r\int_{A_r}^{B_r}E(x,r) G^\prime(x) dx \ll \min \{\frac{\delta\Delta}{T^{1/3}}, T^{2/3+\varepsilon}\delta^{1/2} + T/\delta^{1/2}\}\,.   
% \end{equation}
% All of this allows to replace the internal sum over $n$ with $\int_{A_r}^{B_r} S^\prime(x,r) G(x) dx$. Using the oscillation lemma, we have
% \[
% \sum_r \int_{A_r}^{B_r} S^\prime(x,r) F(T) dx \ll T^{\varepsilon}\Delta\,,
% \]
% Noting that outside of the interval $[A_r,B_r]$ there is no stationary point, and 
% \begin{equation}
%   \int_{\tau}^{X} \brackets{\frac{m}{n}}^{it}e^{i\phi(t)} dt  = \frac{\brackets{\frac{m}{n}}^{it}e^{i\phi(X)}}{\eta(t)}\bigg\vert_{\tau}^{X} + \int_{\tau}^{X} \frac{\brackets{\frac{m}{n}}^{it}e^{i\phi(t)}}{\eta^2(t)} \phi^{\prime\prime}(t) dt  
% \end{equation}
% similarly to the previous lemma the oscillation lemma gives us that the total contribution of this term is of size $\Delta + \delta\Delta^2/T$. Thus the total error is
% \begin{equation}
%   \Delta + T^{5/3}/\Delta + \delta \Delta^2/T + T^{2/3}\delta^{1/2} + \min \{\frac{\delta\Delta}{T^{1/3}}, T/\delta^{1/2}\} \ll \Delta + T^{5/3}/\Delta + \delta \Delta^2/T  
% \end{equation}
% If $\Delta \delta \ll T$, choose $\Delta = T^{5/6}$ with total error $T^{5/6+\varepsilon}$, otherwise $\Delta = T^{8/9}/\delta^{1/3}$ with total error $T^{7/9} \delta^{1/3}$. This expression gives us a non-trivial error term for $\delta \ll T^{2/3}$.

% Finally, expanding $\log m/n$ as $r/x + O(r^2/x^2)$ and using partial integration we have
% \[
% \sum_r \int S(x,r) \frac{T}{x^{2+i\delta}} e^{i\phi(T)}  \brackets{\frac{m}{n}}^{i(T+\beta)} dx = \frac{Te^{i\phi(T)}}{T+\beta} \sum_r \frac{1}{r} \int  e^{i\frac{(T+\beta)r}{x}} \brackets{\frac{S(x,r)}{x^{i\delta}}}^\prime dx\,,
% \]
% which then implies the statement of the lemma.
% \end{proof}



% \begin{proof}
% First, note that
% \[
% \kappa(t) = \exp\brackets{i(t+\alpha)\log \frac{t+\alpha}{2\pi e} - i(t+\beta)\log \frac{t+\beta}{2\pi e}} + O(t^{-1}) = t^{i\delta}+ O(\delta^2/T)\,.
% \]
% Then for $\delta \ll T^{2/5}$ we have
% \begin{eqnarray*}
%   \int_{0}^{T}\brackets{\frac{t}{2\pi}}^{i\delta} \sum_{n\le t/2\pi} \frac{d^2(n)}{n^{1+i\delta}} dt = \frac{T}{2\pi i} \int_{(1)} \frac{\zeta^4(1+s+i\delta)}{\zeta(2+2s+2i\delta)} \brackets{\frac{T}{2\pi}}^{s+i\delta} \frac{ds}{s(1+s+i\delta)} = \\
%   T\brackets{\frac{\zeta^4(1+i\delta)(T/2\pi)^{i\delta}}{(1+i\delta)\zeta(2+2i\delta)} + \res_{s = 0} \frac{\zeta^4(1+s)}{\zeta(2+2s)} \brackets{\frac{T}{2\pi}}^{s} \frac{1}{(s-i\delta)(1+s)}} + O(\sqrt{T} + \delta^2)= \\
%   T\brackets{\frac{\zeta^4(1+i\delta)(T/2\pi)^{i\delta}}{(1+i\delta)\zeta(2+2i\delta)} + \sum_{j=0}^3 \log^j \frac{T}{2\pi} Q_{4-j}(\delta^{-1})} + O(\sqrt{T}+ \delta^2)\,.
% \end{eqnarray*}

% \end{proof}



% \begin{lem}[Off-diagonal term]

% \[
% OD(T;\alpha,\beta) = e^{i\phi(T)} \sum_{r\neq 0} \frac{1}{r} \int  e^{i\frac{(T+\beta)r}{x}} \brackets{\frac{S(x,r)}{x^{i\delta}}}^\prime dx = 
%         \frac{d^2}{ds^2}\brackets{h(\delta,s) \brackets{\frac{(T+\beta) e^{2\gamma_0}}{2\pi}}^s}\,.
% \]
% \end{lem}

% \begin{proof} Recall that the off-diagonal contribution is expressed through
% \begin{equation}
%     e^{i\phi(T)} \sum_{r\neq 0} \frac{1}{r} \int_1^{T/2\pi}  e^{i(T+\beta)\frac{r}{x}} \brackets{\frac{S(x,r)}{x^{i\delta}}}^\prime dx\,.
% \end{equation}
% Change variables to $y = (T+\beta)r/2\pi x$, then the above equals
% \begin{equation}
%     e^{i\phi(T)}\frac{(2\pi)^{i\delta}}{(T+\beta)^{i\delta}}\sum\sum_{r\neq 0} \frac{1}{r^{1+i\delta}} \int_{(T+\beta)r/T}^{(T+\beta)r/2\pi}  e^{2\pi i y} \brackets{S((T+\beta)r/2\pi y,r)y^{i\delta}}^\prime dx\,.
% \end{equation}
% Substituting the expression from Lemma \ref{lem_conrey}, setting $r=mn$ and changing the order of summation and integration we have
% \begin{eqnarray}
%       \sum_{s=1}^{\infty}\frac{\mu(s)}{s^2} \sum_{n =1}^\infty \frac{1}{n^{1+i\delta}} \int_{n}^{\infty} ((u))  \brackets{\frac{1}{u^{1-i\delta}} \brackets{\log^2\frac{(T+\beta) e^{2\gamma_0-1}}{2\pi uns^2}+1}}^\prime du\,.
% \end{eqnarray}
% This then equals
% \begin{eqnarray}
%         \frac{d^2}{ds^2}\brackets{\frac{1}{s+1} \sum_{m\ge 1} \frac{\mu(m)}{m^{2+2s}} \brackets{\frac{(T+\beta) e^{2\gamma_0}}{2\pi}}^s\sum_{n\ge 1}
%         \frac{1}{n^{1+s}} \int_n^{\infty} ((u)) \brackets{\frac{1}{u^{1+s-i\delta}}}^\prime du}= \\
%         \frac{d^2}{ds^2}\brackets{h(\delta,s) \brackets{\frac{(T+\beta) e^{2\gamma_0}}{2\pi}}^s}\,.
% \end{eqnarray}
% \end{proof}
% -------------------------
Now let us move on to the complementary case.

% \newpage
\subsection{Large shifts}
Suppose that $\delta$ is large, in particular, at least as large as a power of $T$. Then one can evaluate
\begin{equation}
  \int\big(\frac{m}{n}\big)^{it} \kappa(t)   W(t) J_{\delta}(nm,t) dt
\end{equation}
using stationary phase analysis similar to Lemma \ref{lem:fresnel}. After obtaining a convenient expression for this integral, one can then use Motohashi's formula for weighted divisor correlations to evaluate the resulting double Dirichlet series.

In this section we consider ``large shifts'' $\delta \gg T^{1/3}$. For this purpose we can set $Q = T^\varepsilon$, and assume that $\delta$ and $\Delta$ satisfy $\delta \Delta^2 \gg \tilde{T}^{2+\varepsilon}$. We will choose optimal $\Delta$ satisfying $(T+\delta)^{1/2+\varepsilon} \ll \Delta \ll T^{1-\varepsilon}$ at the end of the section. Finally, in this section we make the following choice of smoothing:
\begin{equation}
    W(t) = \begin{cases}
    p(|t-T_j|/\Delta), & {|t-T_j| \le \Delta}\,;\\
    % p((2T-t)/\Delta), & {2T - \Delta \le t \le 2T}
    1, & {T_1 + \Delta \le t \le T_2 - \Delta}\,;\\
    0, & \text{otherwise}\,;
    \end{cases}
\end{equation}
where
\[
p(x) = \exp\brackets{-\frac{1}{x} \exp \brackets{-\frac{1}{1-x}}}\,.
\]

Let us start with reducing the off-diagonal contribution to a form compatible with Theorem \ref{thm:moto_exp}. We note that the error term in the following lemma is not optimal in the sense that we effectively gain an extra a factor of $T/\sqrt{\delta}$ by forgoing the spectral expansion analysis for any secondary terms in the stationary phase expansion.
\begin{lem}\label{lem:bigdelta_statphase} Let $W_1(x) := e^{-i\delta \log \delta/2\pi e} \sqrt{2\pi} I(\delta/2\pi r) \delta^{1/2}W(\delta x)$, then
\begin{equation*}
\begin{aligned}
       \sum_{n,m \ge 1} \frac{d(n)d(m)}{n^{1/2}m^{1/2-i\delta}}\int_{-\infty}^{+\infty} \big(\frac{m}{n}\big)^{it} \kappa(t) W(t)  J_{\delta}(nm,t) dt= \\
       \sum_{r=1}^{\infty} \frac{1}{r^{1-i\delta}} \sum_{n,r \ge 1} d(n) d(n+r) W_1(n/r) + O\brackets{\frac{\tilde{T}^{2+\varepsilon}}{\Delta \sqrt{\delta}} + \frac{\delta^{3/2}T^{\varepsilon}}{T}}.
\end{aligned}
\end{equation*}
\end{lem}
\begin{proof}
Let $f(t) = t \log m/n + \phi(t)$, and let $s$ be its stationary point, that is
\begin{equation*}
     f^\prime(s) = \log m/n + \phi^\prime(s) = \log \frac{ms}{n(s+\delta)}=  0\,.
\end{equation*}
Let $r=m-n$, then $s = n\delta/r$, $f^{\prime\prime}(s) = \phi^{\prime\prime}(s)= r^2/(mn\delta)$, and
\[
J_{\delta}(nm,s) = I (\delta/2\pi r) = \frac{1}{2\pi i} \int_{(1)} \brackets{\frac{\delta}{2\pi r}}^{2z} G(z) \frac{dz}{z}\,.
\]
Let $k(u) = k_s(u) = \phi(s+u)- u\phi^{\prime}(s)- \frac{u^2}{2}\phi^{\prime\prime}(s)$, then by Lemma \ref{lem:fresnel}
\begin{equation}
\begin{aligned}
    \int \big(\frac{m}{n}\big)^{it} \kappa(t) W(t) J_{\delta}(nm,t) dt = \big(\frac{m}{n}\big)^{is} \int e^{i\frac{u^2}{2}f^{\prime\prime}(s)}  W(s+u) J_{\delta}(nm,s+u)  e^{ik(u)} du \sim \\
   \sqrt{\pi} e^{i\pi/4} \sum_{j=0}^\infty \frac{(2i)^j (WJe^{ik})^{(2j)}(s)}{j! f(s)^{1/2+j}} = \sqrt{2\pi} e^{if(s) + \pi i/4}\frac{W(s) I(\delta/2\pi r)}{\sqrt{f^{\prime\prime}(s)}} + R_1(m,n)\,.
\end{aligned}
\end{equation}
The term $R_1$ is convergent and is of lower order (hence clearly an error term) when 
\begin{equation}\label{eq:convcond}
  \frac{1}{\Delta^2 f^{\prime\prime}(s)} = \frac{\delta nm}{\Delta^2 r^2} = o(1)\,,  
\end{equation}
in which case
\begin{equation*}
    R_1(m,n) \ll f^{\prime\prime}(s)^{-3/2} (WJ)^{\prime\prime}(s) + f^{\prime\prime}(s)^{-5/2} WJ(s) \phi^{(4)}(s) \,
\end{equation*}
and
\begin{equation*}
    \begin{aligned}
      \sum_{n,m \ge 1} \frac{d(n)d(m)}{n^{1/2}m^{1/2-i\delta}} R_1(m,n) \ll 
      % \delta^{3/2} T^{\varepsilon} \sum_{n,r \ge 1} \frac{n(n+r)}{r^3}\, |(WJ)^{\prime\prime}(n\delta/r) |\ll
      % \frac{T(T+\delta)}{\Delta \sqrt{\delta}} = 
      \frac{\tilde{T}^{2+\varepsilon}}{\Delta \sqrt{\delta}} +\frac{\delta^{3/2}T^{\varepsilon}}{T}\,.
    \end{aligned}
\end{equation*}
In particular, if $s \asymp T$, condition \eqref{eq:convcond} always holds. If \eqref{eq:convcond} does not hold, i.e.
\[
\frac{\delta nm}{\Delta^2 r^2} \gg 1\,,
\]
or $r/n \ll \delta^{1/2}/\Delta \ll \phi^\prime(T)$, then $f(t)$ does not vanish on the support of $WJ$. Let $\eta := \phi^\prime(T)$ and $\eta^\prime := \phi^{\prime\prime}(T)$, then $\min_{t \in [T,2T]} |f^\prime(t)| \gg \eta$ and $\max_{t \in [T,2T]} |f^{\prime\prime}(t)| \ll \eta^\prime$. Integrating by parts $l$ times and applying the oscillation lemma, we see that
\[
\int \big(\frac{m}{n}\big)^{it} \kappa(t) W(t) J_{\delta}(nm,t) dt \ll_l \brackets{\frac{1}{\Delta\eta} + \frac{\sqrt{Q}}{T\eta} + \frac{\eta^\prime}{\eta^2}}^l\max |W(t) J_{\delta}(nm,t)|\,.
\]
Further, with the assumptions we outlined in the beginning of the section,
\[
\frac{1}{\Delta\eta} + \frac{\sqrt{Q}}{T\eta} + \frac{\eta^\prime}{\eta^2} = o(1)\,,
\]
thus the contribution of such $m,n$ is negligible.

This allows us to take as many terms in the asymptotic expansion as necessary so that the remaining series with $j \ge N$ gives an error term as small as desired.
% The first term here can get too large, so let us add it to the main term, such that
% \begin{equation*}
%      \frac{(\delta m n)^{1/2}}{r} W(s) I(\delta/2\pi r) +  \frac{(\delta m n)^{3/2}}{r^3} (WJ)^{\prime\prime}(s)+ R_2(m,n)
% \end{equation*}
% where
% \[
% R_2(m,n) \ll |f^{\prime\prime}(s)|^{-5/2} (WJ)^{(4)}(s)
% \]
% and
% \begin{equation*}
%     \begin{aligned}
%       \sum \frac{d(n)d(m)}{(nm)^{1/2}} R_2(m,n) \ll T^\varepsilon \delta^{5/2} \sum_{n,r} \frac{n^2(n+r)^2}{r^5}(WJ)^{(4)}(s)\ll\\ \delta^{1/2} (T+\alpha)^2(\Delta^{-3} + Q^{3/2}T^{-3})\,.
%     \end{aligned}
% \end{equation*}
% Let
% \[
% W_1(x) = e^{i\delta \log 2\pi e /\delta} \brackets{I(\delta/2\pi r) \delta^{1/2}W(|\delta|x - \alpha) + \delta^{3/2}x(x+1)(WJ)^{\prime\prime}(|\delta|x-\alpha)}\,.
% \]
% Let

Finally, observing that $f(s) +\delta\log m = -\delta \log \delta/2\pi r +\delta$, we then reduce our problem to evaluating
\begin{equation*}
 \sqrt{2\pi} \sum_{n,m \ge 1} \frac{d(n)d(m)}{n^{1/2}m^{1/2-i\delta}} e^{if(s) + \pi i/4}\frac{W(s) I(\delta/2\pi r)}{\sqrt{f^{\prime\prime}(s)}} = 
    \sum_{r=1}^{\infty} \frac{1}{r^{1-i\delta}} \sum_{n,r \ge 1} d(n) d(n+r) W_1(n/r)\,
    \end{equation*}
    as required.
\end{proof}

Now, by Theorem \ref{thm:moto_exp}, for $r \ge 1$
\begin{equation*}
    \sum_{n\ge 1} d(n) d(n+r) W_1(n/r) = \int_0^\infty m(x,r) W_1(x) dx + E(r;W_1)\,,
\end{equation*}
where $E(r;W_1) = e_1(r;W_1) + e_2(r;W_1) + e_3(r;W_1)$ and
\begin{equation*}
\begin{aligned}
      & e_1(r;W_1) = \frac{r^{1/2}}{\pi} \int_{-\infty}^{\infty} \frac{r^{-iy}\sigma_{2iy}(r) |\zeta(1/2+iy)|^4}{|\zeta(1+2iy)|^2} \Theta(y;W_1) dy\,; \\
     &   e_2(r;W_1) = r^{1/2}\sum_{j=1}^{\infty} \alpha_j t_j(r) H_j^2(1/2) \Theta(\kappa_j;W_1)\,; \\
      &  e_3(r;W_1) = \frac{1}{4}r^{1/2} \sum_{k=6}^{\infty} \sum_{j=1}^{\vartheta(k)} (-1)^k \alpha_{j,k} t_{j,k}(r)H_{j,k}^2(1/2) \Xi(k-1/2;W_1)\,.
    \end{aligned}
\end{equation*}

Recall that for a bump function $U(x)$
\begin{equation*}
    \Xi (z;U) =  \frac{\Gamma^2(1/2+z)}{\Gamma(1+2z)} \int_0^\infty U(x) x^{-1/2-z} F(1/2+z,1/2+z,1+2z;-1/x)dx\,,
\end{equation*}
where $F(a,b,c;x)$ is the hypergeometric function, and
\begin{equation*}
    \Theta(y;U) = \frac{1}{2} \re \brackets{ \brackets{1 + \frac{i}{\sinh{\pi y}}} \Xi(iy;U)}\,.
\end{equation*}
Note that $\Xi(y;W_1)$ and $\Theta(y;W_1)$ do not depend on $r$ at all, while the $\sum_r e_j(r;W_1)/r^{1-i\delta}$ turn out to be absolutely convergent as double sums. To see that, let us first bound $\Xi(y;W_1)$ and $\Theta(y;W_1)$.

\begin{lem} \label{lem:thetaxi} Let $W_2(x) = \delta^{1/2}W(\delta x)$. Then for $y \in \RR$ and any $l \in \NN$
\[
\Xi(iy;W_2) \ll_l \frac{\tilde{T}^{l+1/2}}{(1 + |y|)^{l+3/2} \Delta^l}, \ \Theta(y;W_2) \ll  \frac{\tilde{T}^{1/2}(1 + 1/y)}{(1 + |y|)^{3/2}}\,.
\]
In addition, for $k \in \NN$
\[
    \Xi(k-1/2;W_2) \ll \delta^{1/2}\begin{cases}
    \frac{(k-1)!^2}{(2k-1)!} \brackets{\frac{\delta}{T}}^{k-1}, & \text{if $\delta \le T$}\,;\\
    \min\{\frac{1}{k^2}, \frac{1}{k} e^{-Ck\sqrt{T/\delta}}\}, & \text{otherwise}\,.
    \end{cases}
\]
\end{lem}
\begin{proof}
By definition,
\begin{equation*}
    \Xi(iy;W_2) = \int_0^\infty W_2(x) \int_0^1 (w(1-w))^{-1/2+iy} (x+w)^{-1/2-iy} dw dx\,,
\end{equation*}
and integrating by parts $l+1$ times with respect to $x$ gives
\begin{equation*}
    \Xi(iy;W_2) \ll_l (1 + |y|)^{-l-1} \bigg\vert \int_0^\infty W_2^{(l+1)}(x) dx  \int_0^1 (w(1-w))^{-1/2+iy} (x+w)^{l+1/2-iy} dw\bigg\vert\,.
\end{equation*}
We can bound the internal integral using the oscillation lemma for the second derivative, which is slightly different depending on whether $|x| \ll 1$ or $|x| \gg 1$. The stationary point of $y \log(w/(1-w) - y \log (x+w)$ is at $w_s = \sqrt{x^2+x} - x$, hence
\begin{equation*}
    \int_0^1 (w(1-w))^{-1/2+iy} (x+w)^{l+1/2-iy} dw \ll (1+|y|)^{-1/2} \min\{|x|,|x|^{1/2}\}^{l+1/2}\,.
\end{equation*}
Using the trivial upper bound for the integrand,
\begin{equation*}
\begin{aligned}
 &  \Xi(iy;W_2) \ll_l (1 + |y|)^{-l-3/2} \int_0^\infty |W_2^{(l+1)}(x)| \min\{|x|,|x|^{1/2}\}^{l+1/2} dx \ll_l \\
  & \frac{\delta^{l+1/2}}{(1 + |y|)^{l+3/2} \Delta^l} \min\{T/\delta,\sqrt{T/\delta}\}^{l+1/2} \ll_l \frac{\tilde{T}^{l+1/2}}{(1 + |y|)^{l+3/2} \Delta^l}\,.
\end{aligned}
\end{equation*}
In particular, this implies that we can restrict to $y \ll X^{1+\varepsilon}$, where
\[
X= X(T,\delta,\Delta) := \tilde{T}/\Delta\,,
\]
and take $l=0$. A similar bound to above applies to $\Theta(y;W_2)$ with
\begin{equation}\label{eq:Thetabound}
  \Theta(y;W_2)  = \frac{1}{2} \re \brackets{ \brackets{1 + \frac{i}{\sinh{\pi y}}} \Xi(iy;W_2)} \ll  \frac{\tilde{T}^{1/2}(1 + 1/y)}{(1 + |y|)^{3/2}}\,. 
\end{equation}
When $z = k-1/2$ and $k \in \NN$, we have
\begin{equation}\label{eq:Xibound}
    \Xi(k-1/2;W_2) \ll \delta^{1/2}\begin{cases}
    \frac{(k-1)!^2}{(2k-1)!} \brackets{\frac{\delta}{T}}^{k-1}, & \text{if $\delta \le T$}\,,\\
    \min\{\frac{1}{k^2}, \frac{1}{k} e^{-Ck\sqrt{T/\delta}}\}, & \text{otherwise}\,,
    \end{cases}
\end{equation}
where $C>0$ is fixed. The first case follows directly from the series representation of the hypergeometric function. The second case follows after integrating by parts as above and observing that for $w \in (0,1)$ and $x \asymp T/\delta < 1$
\[
\frac{w(1-w)}{x+w} = \frac{1-w}{1+x/w} = \exp \brackets{\log \frac{1-w}{1+x/w}}\le \begin{cases}
e^{-C_1(w+ x/w)}, & \text{if $ w > x$}\,;\\
e^{-C_2 (w + w/x + \log w/x)}, & \text{if $ w \le x$}\,.
\end{cases}
\]
In both cases, this is $O(e^{-C_3\sqrt{x}})$ with some fixed constants $C_j>0$.
\end{proof}

These bounds together with the weight $I(\delta/2\pi r)$ for the sum over $r$ implies that sums $\sum e_j(r,W_1)/r^{1-i\delta}$ are indeed absolutely convergent since they are essentially truncated in both variables. This means that by Fubini's theorem we can freely change the order of summation (and integration). Now let us use Lemma \ref{lem:thetaxi} to bound the contribution of the error term in Motohashi's theorem. We note that the bound here essentially depends on the best sub-convexity bounds known for $\zeta(1/2+it)$ as well as Hecke $L$-functions $H_j(1/2+it)$ and $H_{j,k}(1/2+it)$.

\begin{lem}\label{lem:bigdelta_correr} Let $E(r;W_1) = e_1(r;W_1) + e_2(r;W_1) + e_3(r;W_1)$, where
\begin{equation*}
    \begin{aligned}
       & e_1 = \frac{r^{1/2}}{\pi} \int_{-\infty}^{\infty} \frac{r^{-iy}\sigma_{2iy}(r) |\zeta(1/2+iy)|^4}{|\zeta(1+2iy)|^2} \Theta(y;W_1) dy\,;\\
       & e_2 =  r^{1/2}\sum_{j=1}^{\infty} \alpha_j t_j(r) H_j^2(1/2) \Theta(\kappa_j;W_1)\,;\\
       & e_3 = \frac{1}{4}r^{1/2} \sum_{k=6}^{\infty} \sum_{j=1}^{\vartheta(k)} (-1)^k \alpha_{j,k} t_{j,k}(r)H_{j,k}^2(1/2) \Xi(k-1/2;W_1)\,.
    \end{aligned}
\end{equation*}
Then 
\[
\sum_{r \ge 1} \frac{E(r;W_1)}{r^{1-i\delta}} \ll \frac{\tilde{T}^{1+\varepsilon}}{\Delta^{1/2}} + \tilde{T}^{1/2+\varepsilon}\delta^{1/3} +  \delta^{5/6+\varepsilon}.
\]
\end{lem}
\begin{proof}
Let $E_j = \sum_{r \ge 1} e_j(W_1,r)/r^{1-i\delta}$ for $j = 1,2,3$. Recall that
\[
W_1(x) = e^{i\delta \log 2\pi e /\delta} I(\delta/2\pi r) \delta^{1/2}W(\delta x) = e^{i\delta \log 2\pi e /\delta} I(\delta/2\pi r) W_2(x)\,,
\]
so the error terms factorise conveniently. Let 
\begin{equation*}
    \begin{aligned}
      & Z_{iy}(1/2+it) = e^{it \log 2\pi e /t}\sum_{r=1}^\infty \frac{\sigma_{2iy}(r)I(|t|/2\pi r)}{r^{1/2+it+iy}} \,;\\
    & L_j(1/2+it) := e^{it \log 2\pi e /t}\sum_{r=1}^\infty \frac{t_j(r)I(|t|/2\pi r)}{r^{1/2+it}}\,;\\
       & L_{j,k}(1/2+it): =  e^{it \log 2\pi e /t} \sum_{r=1}^\infty \frac{t_{j,k}(r)I(|t|/2\pi r)}{r^{1/2+it}} \,.
    \end{aligned}
\end{equation*}
As $I(|t|/2\pi r)$ is just a weight function essentially truncating the sum at $r \le |t|/2\pi$, the functions above are approximations of $\zeta(1/2 + t+iy)\zeta(1/2+it-iy)$, $H_j(1/2+it)$ and $H_{j,k}(1/2+it)$ respectively. Changing the order of summation and integration due to absolute convergence, we then have
\begin{equation*}
    \begin{aligned}
   & E_1 = \frac{1}{\pi} \int_{-\infty}^{\infty} \frac{Z_{iy}(1/2-i\delta) |\zeta(1/2+iy)|^4}{|\zeta(1+2iy)|^2} \Theta(y;W_2) dy\,;\\
     &   E_2 = \sum_{j=1}^{\infty} \alpha_j L_j(1/2-i\delta) H_j^2(1/2) \Theta (\kappa_j;W_2)\,;\\
    &   E_3 = \frac{1}{4} \sum_{k=6}^{\infty} \sum_{j=1}^{\vartheta(k)} (-1)^k \alpha_{j,k} L_{j,k}(1/2-i\delta) t_{j,k}(r)H_{j,k}^2(1/2) \Xi(k-1/2;W_2)\,.
    \end{aligned}
\end{equation*}
Let us first bound $E_1$. Applying \eqref{eq:Thetabound},
\begin{equation*}
\begin{aligned}
   E_1 \ll \tilde{T}^{1/2} \int_{y \ll X^{1+\varepsilon}} \frac{|Z_{iy}(1/2+i\delta)| |\zeta(1/2+iy)|^4(1+1/|y|)}{|\zeta(1+2iy)|^2(1+|y|)^{3/2}}  dy \,,
       \end{aligned}
\end{equation*}
so it remains to bound $Z_{iy}(1/2+i\delta)$. Recall the subconvexity bound 
\begin{equation}\label{eq:zeta_upperbound}
    \zeta(1/2+it) \ll (1+|t|)^{13/84+\varepsilon} \ll (1+|t|)^{1/6}\,.
\end{equation}
The approximate functional equation for the Riemann zeta implies that
\[
|\zeta(1/2+it)|\le 2 \bigg\vert\sum_{n \le \sqrt{t/2\pi}} n^{-1/2-it}\bigg\vert + O(1)\,,
\]
and in fact, going back to the proof \cite{bourgain2017decoupling}, the bound \eqref{eq:zeta_upperbound} is a consequence of a corresponding bound for exponential sums $\sum_{n \le N} e^{-it\log n}$. Similarly in our case, $Z_{iy}(1/2+i\delta)$ has the same upper bound. 

Let us give a quick proof of this fact. Recall the definition of $I(w)$, then
\begin{equation*}
    \sum_{r=1}^\infty \frac{\sigma_{2iy}(r)I(|t|/2\pi r)}{r^{1/2+it+iy}} = \frac{1}{2\pi i} \int_{(1)} \zeta(1/2+it+iy+s)\zeta(1/2+it-iy+s) \brackets{\frac{|t|}{2\pi}}^s G(s) \frac{ds}{s}\,.
\end{equation*}
Moving the line of integration to $(0)$ with a small semi-circle around $(0)$ we pick up poles at $s=1/2-it \pm iy$ with residues
\[
\zeta(1\pm 2iy) \brackets{\frac{|t|}{2\pi}}^{1/2-it\pm iy}  \frac{G(1/2-it \pm iy)}{1/2-it \pm iy} \ll  \frac{|t|^{1/2}}{1+|t \pm y|}|\zeta(1\pm 2iy)| G(i|t\pm y|)
\]
as well as half the pole at $s=0$ with residue $\zeta(1/2+it+iy)\zeta(1/2+it-iy)$. Finally,
\begin{equation*}
\begin{aligned}
    \int_{|w| \ge 1} \zeta(1/2+it+iy+iw)\zeta(1/2+it-iy+iw) \brackets{\frac{|t|}{2\pi}}^{iw} G(iw) \frac{dw}{w} \ll \\
    \int_{1\ll |w| \ll Q^{1/2}T^{\varepsilon}} |\zeta(1/2+it+iy+iw)\zeta(1/2+it-iy+iw)| \frac{dw}{w}\,.
\end{aligned}
\end{equation*}
Thus if $|t\pm y| \gg Q^{1/2}T^{\varepsilon} \gg T^{\varepsilon}$, the bound \eqref{eq:zeta_upperbound} applies to $Z_{iy}(1/2+it)$. Otherwise we have the trivial bound $Z_{iy}(1/2+it) \ll |t|^{1/2+\varepsilon}$.

Using this bound together with $\zeta(1+it) \gg 1 + 1/|t|$ and $\int_0^N |\zeta(1/2+it)|^4dt \ll N^{1+\varepsilon}$,
\begin{equation*}
    \begin{aligned}
       & \int_{|\delta \pm y| \gg Q^{1/2}T^{\varepsilon}} \frac{|Z_{iy}(1/2+i\delta)| |\zeta(1/2+iy)|^4(1+1/|y|)}{|\zeta(1+2iy)|^2(1+|y|)^{3/2}}  dy \ll \\
       & \int_{|\delta \pm y| \gg Q^{1/2}T^{\varepsilon}} \frac{|\delta^2-y^2|^{1/6} |\zeta(1/2+iy)|^4}{(1+|y|)^{3/2}}  dy \ll
        \delta^{1/3+\varepsilon}\,
    \end{aligned}
\end{equation*}
and
\begin{equation*}
    \begin{aligned}
        \int_{|\delta \pm y| \ll Q^{1/2}T^{\varepsilon}} \frac{|Z_{iy}(1/2+i\delta)| |\zeta(1/2+iy)|^4(1+1/|y|)}{|\zeta(1+2iy)|^2(1+|y|)^{3/2}}  dy \ll \\
      \frac{1}{\delta} \int_{|\delta \pm y| \ll Q^{1/2+\varepsilon}} \frac{ |\zeta(1/2+iy)|^4}{|\zeta(1+2iy)|}  dy \ll
        T^{\varepsilon}\,.
    \end{aligned}
\end{equation*}
Thus
\begin{equation*}
    \begin{aligned}
   E_1 \ll \tilde{T}^{1/2} \int_{y \ll X^{1+\varepsilon}} \frac{|Z_{iy}(1/2+i\delta)| |\zeta(1/2+iy)|^4(1+1/|y|)}{|\zeta(1+2iy)|^2(1+|y|)^{3/2}}  dy \ll  \tilde{T}^{1/2+\varepsilon}\delta^{1/3}\,.
%   \frac{\tilde{T}^{1/2}|\delta + X|^{1/3}}{X^{1/2}}\ll
%     \Delta^{1/3} |\delta|^{1/3} + \Delta^{1/6}\tilde{T}^{1/3}\,;\\
    \end{aligned}
\end{equation*}
% \begin{equation*}
%     \begin{aligned}
%       &Z_{iy}(1/2+i\delta) \ll
%     |\delta + y|^{1/6+\varepsilon}|\delta - y|^{1/6+\varepsilon}\,;\\
%     & L_j(1/2+i\delta) \ll
%          |\delta + \kappa_j|^{1/3+\varepsilon}\,;\\
%       & L_{j,k}(1/2+i\delta) \ll |\delta + k|^{1/3+\varepsilon}\,,
%     \end{aligned}
% \end{equation*}
% In particular, for $\zeta$ we used a subconvexity result $\zeta(1/2+it) \ll t^{1/6}$, which is worse than one obtained by Bourgain \cite{bourgain2017decoupling}, but it suffices for our purposes here. All bounds apply to both $L$-functions and their weighted approximations. 
To bound $E_2$ and $E_3$ we will use bounds from Lemma \ref{lem:Sjmoment}. Same bounds apply if one replaces $S_j$ and $S_{j,k}$ with $L_j$ and $L_{j,k}$ respectively via a standard partial summation argument, thus we also have
\begin{equation}\label{eq:Sjmoment2}
\begin{aligned}
  &  \sum_{K \le \kappa_j \le 2K} \alpha_j |L_j(1/2+it)|^2 \ll K^{2+\varepsilon} + K^{\varepsilon}t^{2/3+\varepsilon}\,,\\
   &     \sum_{K \le k \le 2K} \sum_{j=1}^{\vartheta (k)} \alpha_{j,k}|L_{j,k}(1/2+it)|^2 \ll K^{2+\varepsilon} + K^{\varepsilon}t^{2/3+\varepsilon}\,.
\end{aligned}
\end{equation}
Plugging \eqref{eq:Thetabound} into $E_2$, and using Cauchy's inequality,
\begin{equation*}
\begin{aligned}
    E_2 \ll  \tilde{T}^{1/2}\sum_{\kappa_j \ll X^{1+\varepsilon}} & \frac{\alpha_j |L_j(1/2+i\delta)| H_j^2(1/2)}{\kappa_j^{3/2}} \ll \\ & \tilde{T}^{1/2}\sqrt{\sum_{\kappa_j \ll X^{1+\varepsilon}}\frac{\alpha_j |L_j(1/2+i\delta)|^2}{ \kappa_j} \sum_{\kappa_j \ll X^{1+\varepsilon}}\frac{\alpha_j H_j^4(1/2)}{\kappa_j^{2}}}\,.
    \end{aligned}
\end{equation*}
Split the sums into dyadic intervals. Applying \eqref{eq:Hjmoment} to the first sum then gives
\[
\sum_{\kappa_j \ll X^{1+\varepsilon}}\alpha_j H_j^4(1/2)\kappa_j^{-2} \ll X^{\varepsilon}\,,
\]
while \eqref{eq:Sjmoment2} similarly gives
\[
\sum_{\kappa_j \le X^{1+\varepsilon}}\alpha_j \kappa_j^{-1} |L_j(1/2+i\delta)|^2 \ll X^{1+\varepsilon} + \delta^{2/3+\varepsilon} X^{\varepsilon}\,.
\]
Thus, substituting $X = \tilde{T}/\Delta$,
\[
 E_2  \ll
   \tilde{T}^{1+\varepsilon}/\Delta^{1/2} + \tilde{T}^{1/2+\varepsilon}\delta^{1/3}\,.
\]
Similarly for $E_3$, if $\delta \le T$, applying the first case in \eqref{eq:Xibound} together with \eqref{eq:Sjmoment2}, and then Cauchy's inequality,
\begin{equation*}
    \begin{aligned}
   E_3 \ll \delta^{1/2} \brackets{\frac{\delta}{T}}^5 \sum_{6 \le k \le X^{1+\varepsilon}} \sum_{j=1}^{\vartheta(k)} \alpha_{j,k} |L_{j,k}(1/2+i\delta)| H_{j,k}^2(1/2) 2^{-k}\,\ll
%   \frac{\delta^{5+5/6+\varepsilon}}{(T+\alpha)^5} \ll 
   \delta^{5/6+\varepsilon} \,.
    \end{aligned}
\end{equation*}
If $\delta > T$, then applying the second case in \eqref{eq:Xibound} instead,
\begin{equation*}
    \begin{aligned}
   E_3 \ll \delta^{1/2}  \sum_{6 \le k \ll T^{\varepsilon}\sqrt{\frac{\delta}{T}}} \sum_{j=1}^{\vartheta(k)}  \alpha_{j,k} |L_{j,k}(1/2+i\delta)| H_{j,k}^2(1/2) k^{-2} \ll 
   \delta^{5/6+\varepsilon}\,.
    \end{aligned}
\end{equation*}
Thus the total error is
\[
E_1 + E_2 + E_3 \ll \tilde{T}^{1+\varepsilon}/\Delta^{1/2} + \tilde{T}^{1/2+\varepsilon}\delta^{1/3} +  \delta^{5/6+\varepsilon}\,.
\]
In particular, this restricts us to $\delta \ll T^{6/5-\varepsilon}$. 
\end{proof}

Finally, let us evaluate the main term given by
\begin{equation}\label{eq:bigdelta_main}
     \sum_{r=1}^{\infty} \frac{1}{r^{1-i\delta}} \int_0^{\infty} m(x,r) W_1(\delta x) dx\,,
\end{equation}
and confirm that it coincides with the Motohashi formula.

\begin{lem}Let
\[
h(z,s)= \frac{\zeta(1+z+s)\zeta(1-z+s)}{\zeta(2+2s)}\,,
\]
and
\[
 H_{\delta}(t) = \frac{d^2}{ds^2}\, \brackets{h(i\delta,s) \frac{t^{s/2}(t+\delta)^{s/2}}{(2\pi)^s}e^{2\gamma_0 s}} \bigg\vert_{s=0} - \frac14 h(i\delta,0) \log^2 \frac{t}{t+\delta}\,.
 \]
 Then
\[
2 \re \sum_{r=1}^{\infty} \frac{1}{r^{1-i\delta}} \int_0^{\infty} m(x,r) W_1(\delta x) dx = \int_0^\infty W(t)  H_{\delta}(t) (1+ O(\delta^{-1/2+\varepsilon})) dt\,.
\]
\end{lem}
\begin{proof}
Recall the definition of $I(w)$, then changing the order of summation and integration due to absolute convergence, and summing over $r$, we have
\begin{equation}\label{eq:mxrseries}
    \sum_{r=1}^{\infty} \frac{m(x,r)}{r^{1-i\delta}}I(\delta/2\pi r) = \frac{1}{2\pi i} \int_{(2)} L(x, 1- i\delta + s) \brackets{\frac{\delta}{2\pi}}^s \frac{G(s/2)}{s}ds\,,
\end{equation}
where $ L(x, 1+z) = \lim_{h\to 0} L_h(x,1+z)$ and
\begin{eqnarray*}
        L_h(x,1+z) = \frac{\zeta^2(1+ h)}{\zeta(2+2h)} \zeta(1+z)\zeta(z-2h)x^h (1 + x)^h + \frac{\zeta^2(1- h)}{\zeta(2-2h)} \zeta(1+z-2h)\zeta(z) + \\ \frac{\zeta(1+h)\zeta(1-h)}{\zeta(2)}\zeta(1+z-h)\zeta(z-h)(x^h + (1+ x)^h) \,.
\end{eqnarray*}
Moving the line of integration to $\re s = 0$ with a small half-circle around $0$ gives $1/2$ of the residue at $0$, and residues at $s=\pm i\delta$, thus \eqref{eq:mxrseries} equals
\begin{equation}
   \frac{1}{2} L(x,1-i\delta) + O(e^{-\delta^2/4Q}) + \frac{1}{2\pi i} \int_{|\Im s| \ge a} L(x, 1- i\delta + s) \brackets{\frac{\delta}{2\pi}}^s \frac{G(s)}{s}ds\,.
\end{equation}
Similarly to \eqref{eq:intrealpart} in Theorem \ref{thm:odsmall} observe that 
\begin{equation*}
   \re \frac{1}{2\pi i} \int_{|y| \ge a} L(x, 1- i\delta + s) \brackets{\frac{\delta}{2\pi}}^{iy} \frac{G(iy)}{y}dy \ll \frac{Q T^{\varepsilon}}{\delta^{1/2}}\ll \delta^{-1/2+\varepsilon}\,.
\end{equation*}
Finally, changing variables to $t = \delta x$ in
\eqref{eq:bigdelta_main} we see that $L(x,1-i\delta) = H_{\delta}(t)$, which then implies the statement of the lemma.
\end{proof}

\begin{thm}[Off-diagonal term]\label{thm:odbig} 
% Let $W$ be an infinitely differentiable function supported on $[T,2T]$ chosen with parameter $\Delta$.
Let $0\le \delta \ll T^{8/5}$. Set $\tilde{T} :=\sqrt{T(T+\delta)}$ and $Q = T^\varepsilon$. Additionally, assume that $\delta \Delta^2 \gg \tilde{T}^{2+\varepsilon}$. Finally, let
\[
h(z,s)= \frac{\zeta(1+z+s)\zeta(1-z+s)}{\zeta(2+2s)}\,,
\]
and
\[
 H_{\delta}(t) = \frac{d^2}{ds^2}\, \brackets{h(i\delta,s) \frac{t^{s/2}(t+\delta)^{s/2}}{(2\pi)^s}e^{2\gamma_0 s}} \bigg\vert_{s=0} - \frac14 h(i\delta,0) \log^2 \frac{t}{t+\delta}\,.
 \]
Then
\begin{equation*}
    \begin{aligned}
      2 \re\sum_{n \neq m} \frac{d(n)d(m)}{n^{1/2}m^{1/2-i\delta}} \int\big(\frac{m}{n}\big)^{it} \kappa(t)  W(t)  V_{\delta}(nm,t) dt =  \int W(t)  H_{\delta}(t)dt+ \\
    %   \delta^{1/2} (T+\alpha)\brackets{\frac{1}{\Delta} + \frac{Q^{1/2}}{T}} + ((T+\alpha)(T+\beta)\Delta^{-1})^{1/2} + \Delta^{1/2}\delta^{1/3} +\\ (\Delta(T+\alpha)(T+\beta))^{1/6} + \frac{\delta^{3/2}Q^{1/2}}{T+\beta} + \frac{\delta^{1/2} Q}{T+\alpha}
    O\brackets{
   \frac{\tilde{T}^2}{\Delta \sqrt{\delta}} + \delta^{5/6+\varepsilon} + \frac{\delta^{3/2}T^{\varepsilon}}{T} + \delta^{1/3+\varepsilon}\tilde{T}^{1/2+\varepsilon}}\,.
    \end{aligned}
\end{equation*}
% In particular, if $\beta \ll T$
% \[
%  \frac{\delta^{1/2}T}{\Delta} + \frac{\delta^{3/2}Q^{1/2}}{T} + \Delta^{1/2}\delta^{1/3} + T^{2/3}
% \]
% otherwise
% \[
% \delta^{1/2} \frac{T+\alpha}{\Delta} + \brackets{\frac{(T+\alpha)\beta}{\Delta}}^{1/2} + (\delta Q)^{1/2} +   \Delta^{1/2}\delta^{1/3} + T^{2/3}\,.
% \]
% If $\alpha \ll T$ this is
% \[
%  \frac{T\beta^{1/2}}{\Delta} + \brackets{\frac{T\beta}{\Delta}}^{1/2} + (\beta Q)^{1/2} +   \Delta^{1/2}\beta^{1/3} + T^{2/3}
% \]
In particular, $\Delta = \tilde{T}^{1-\varepsilon}/\delta^{1/4}$ gives error term of size
\[
\frac{\tilde{T}^{1+\varepsilon}}{\delta^{1/4}} + \delta^{5/6+\varepsilon} + \delta^{1/3+\varepsilon}\tilde{T}^{1/2+\varepsilon}\, = o(T)
\]
when $\delta \ll T^{6/5-\varepsilon}$ and $(T+\alpha)(T+\beta) \ll T^{2-\varepsilon} \delta^{1/2}$.
\end{thm}

\begin{proof}

The error term follows after collecting errors from Lemma \ref{lem:sweights}, \ref{lem:bigdelta_statphase} and \ref{lem:bigdelta_correr} with total
\[
  \frac{\tilde{T}^2}{\Delta \sqrt{\delta}} + \frac{\tilde{T}^{1+\varepsilon}}{\Delta^{1/2}} +  \delta^{1/2+\varepsilon} + \frac{T+\beta}{\delta^{1/2}} +
    % \Delta^{1/2}\delta^{1/3} + T^{2/3}\,.
     \delta^{1/3}(T+\beta)^{1/2+\varepsilon} \ll   \frac{\tilde{T}^2}{\Delta \sqrt{\delta}} +
     \delta^{1/3}(T+\beta)^{1/2+\varepsilon}\,.
\]
This concludes the proof.
\end{proof}

\subsection{Diagonal term and main theorem}
To conclude our computation, let us finally evaluate the diagonal term.


Putting together Theorems \ref{thm:diag}, \ref{thm:odsmall} and \ref{thm:odbig}, and summing over dyadic intervals yields Theorem \ref{thm:A}. Since $\alpha$ and $\beta$ are fixed, and $T$ varies, we apply the appropriate version of the main theorem to each range. Note that when $T^{1/3} \ll \delta \ll T^{1/2-\varepsilon}$, the bound from Theorem \ref{thm:odbig} is better than the one in Theorem \ref{thm:odsmall}. If $E(X)$ is the error term on the interval $[X,2X]$ and $\tilde{X} = \sqrt{(X+\alpha)(X+\beta)}$, then
\[
E(X) \ll X^{\varepsilon} \begin{cases}
\tilde{X}^{4/5}, & \text{if $\delta \ll \tilde{X}^{1/3}$}\,;\\
\frac{\tilde{X}}{\delta^{1/4}} + \delta^{1/3}\tilde{X}^{1/2} + \delta^{5/6}, & \text{if $\delta \gg \tilde{X}^{1/3}$}\,.
\end{cases}
\]
Thus
\[
\sum_{j \le \log T} E(T/2^j) \ll T^{\varepsilon} \begin{cases}
\tilde{T}^{4/5} + \delta^{11/4}, & \text{if $\delta \ll T^{1/3}$}\,;\\
\frac{\tilde{T}}{\delta^{1/4}} + \delta^{1/3}\tilde{T}^{1/2} + \delta^{5/6}, & \text{otherwise}\,.
\end{cases}
\]
In particular, this is bounded by $O((T+\alpha)^{11/12+\varepsilon} + \delta^{5/6+\varepsilon})$. This bound is not optimal, and can be further improved by doing the stationary phase analysis more carefully, except for the biggest contribution coming from $E_2$ and $E_3$ in Lemma \ref{lem:bigdelta_correr}.
